The Dresden in-situ (S)TEM special with a continuous-flow liquid-helium cryostat

Fundamental solid state physics phenomena typically occur at very low temperatures, requiring liquid helium cooling in experimental studies. Transmission electron microscopy is a well-established characterization method, which allows probing crucial materials properties down to nanometer and even atomic resolution. Due to the limited space in the object plane, however, suitable liquid-helium cooling is very challenging. To overcome this limitation, resolving power was sacrificed in our Dresden in-situ (S)TEM special, resulting in more than 60 mm usable experimental space in all directions with the specimen in the center. With the installation of a continuous-flow liquid-helium cryostat, any temperature between 6.5 K and 400 K can be set precisely and kept for days. The information limit of the Dresden in-situ (S)TEM special is about 5 nm. It is shown that the resolution of the Dresden in-situ (S)TEM special is currently not limited by aberrations, but by external instabilities, that are currently addressed.

==> figures/cetcor/cetcor_old.tex <==
\definecolor{cb4b6b9}{RGB}{180,182,185}
\definecolor{c211e1f}{RGB}{33,30,31}
\definecolor{c77797b}{RGB}{119,121,123}
\def\y1{0.5}
\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-\y1, xscale=1.000000, inner sep=0pt, outer sep=0pt]
	\begin{scope}[cm={{2.062,0.0,0.0,-2.062,(-129.99548,1482.0161)}}]
	
%ol
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (280.9290,626.1980) .. controls					
	(280.9290,618.7370) and (252.3650,612.6880) .. (229.4670,612.6880) .. controls
	(206.5680,612.6880) and (178.0060,618.7370) .. (178.0060,626.1980) .. controls
	(178.0060,633.6590) and (206.5680,639.7080) .. (229.4670,639.7080) .. controls
	(252.3650,639.7080) and (280.9290,633.6590) .. (280.9290,626.1980);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line width=0.400pt] 
(280.9290,626.1980) .. controls (280.9290,618.7370) and
(252.3650,612.6880) .. (229.4670,612.6880) .. controls (206.5680,612.6880) and
(178.0060,618.7370) .. (178.0060,626.1980) .. controls (178.0060,633.6590) and
(206.5680,639.7080) .. (229.4670,639.7080) .. controls (252.3650,639.7080) and
(280.9290,633.6590) .. (280.9290,626.1980) -- cycle;


\path[fill=cb4b6b9,nonzero rule] (283.7750,586.0280) .. controls
(283.7750,582.2590) and (248.4730,579.2040) .. (229.5980,579.2040) .. controls
(210.7230,579.2040) and (175.4200,582.2590) .. (175.4200,586.0280) .. controls
(175.4200,589.7960) and (210.7230,592.8500) .. (229.5980,592.8500) .. controls
(248.4730,592.8500) and (283.7750,589.7960) .. (283.7750,586.0280);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.7750,586.0280) .. controls (283.7750,582.2590) and
(248.4730,579.2040) .. (229.5980,579.2040) .. controls (210.7230,579.2040) and
(175.4200,582.2590) .. (175.4200,586.0280) .. controls (175.4200,589.7960) and
(210.7230,592.8500) .. (229.5980,592.8500) .. controls (248.4730,592.8500) and
(283.7750,589.7960) .. (283.7750,586.0280) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.0290,532.5260) .. controls
(283.0290,528.8980) and (248.7270,525.9580) .. (229.8510,525.9580) .. controls
(210.9750,525.9580) and (175.6740,528.8980) .. (175.6740,532.5260) .. controls
(175.6740,536.1530) and (210.9750,539.0930) .. (229.8510,539.0930) .. controls
(248.7270,539.0930) and (283.0290,536.1530) .. (283.0290,532.5260);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.0290,532.5260) .. controls (283.0290,528.8980) and
(248.7270,525.9580) .. (229.8510,525.9580) .. controls (210.9750,525.9580) and
(175.6740,528.8980) .. (175.6740,532.5260) .. controls (175.6740,536.1530) and
(210.9750,539.0930) .. (229.8510,539.0930) .. controls (248.7270,539.0930) and
(283.0290,536.1530) .. (283.0290,532.5260) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.9060,472.3160) .. controls
(283.9060,468.6220) and (248.6320,465.6260) .. (229.7890,465.6260) .. controls
(210.9470,465.6260) and (175.6720,468.6220) .. (175.6720,472.3160) .. controls
(175.6720,476.0110) and (210.9470,479.0060) .. (229.7890,479.0060) .. controls
(248.6320,479.0060) and (283.9060,476.0110) .. (283.9060,472.3160);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,472.3160) .. controls (283.9060,468.6220) and
(248.6320,465.6260) .. (229.7890,465.6260) .. controls (210.9470,465.6260) and
(175.6720,468.6220) .. (175.6720,472.3160) .. controls (175.6720,476.0110) and
(210.9470,479.0060) .. (229.7890,479.0060) .. controls (248.6320,479.0060) and
(283.9060,476.0110) .. (283.9060,472.3160) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.9060,432.8440) .. controls
(283.9060,429.1500) and (248.6320,426.1550) .. (229.7890,426.1550) .. controls
(210.9470,426.1550) and (175.6720,429.1500) .. (175.6720,432.8440) .. controls
(175.6720,436.5390) and (210.9470,439.5350) .. (229.7890,439.5350) .. controls
(248.6320,439.5350) and (283.9060,436.5390) .. (283.9060,432.8440);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,432.8440) .. controls (283.9060,429.1500) and
(248.6320,426.1550) .. (229.7890,426.1550) .. controls (210.9470,426.1550) and
(175.6720,429.1500) .. (175.6720,432.8440) .. controls (175.6720,436.5390) and
(210.9470,439.5350) .. (229.7890,439.5350) .. controls (248.6320,439.5350) and
(283.9060,436.5390) .. (283.9060,432.8440) -- cycle;
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,391.8650) .. controls
(283.9060,388.1700) and (248.6320,385.1750) .. (229.7890,385.1750) .. controls
(210.9470,385.1750) and (175.6720,388.1700) .. (175.6720,391.8650) .. controls
(175.6720,395.5590) and (210.9470,398.5550) .. (229.7890,398.5550) .. controls
(248.6320,398.5550) and (283.9060,395.5590) .. (283.9060,391.8650);


\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,391.8650) {ADL};
\node[color=red!80!black, anchor=base west, yshift=6*\y1, xshift=5] at (286.9230,406.0820) {HP2};
\node[color=red!80!black, anchor=base west, yshift=8*\y1, xshift=5] at (286.9230,486.2910) {HP1};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,432.8440) {TL22};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,472.3160) {Tl21};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,532.5260) {TL12};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,586.0280) {TL11};

\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,322.0650) {SAD plane};
\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,626.0810) {specimen plane};


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,391.8650) .. controls (283.9060,388.1700) and
(248.6320,385.1750) .. (229.7890,385.1750) .. controls (210.9470,385.1750) and
(175.6720,388.1700) .. (175.6720,391.8650) .. controls (175.6720,395.5590) and
(210.9470,398.5550) .. (229.7890,398.5550) .. controls (248.6320,398.5550) and
(283.9060,395.5590) .. (283.9060,391.8650) -- cycle;
\path[fill=c77797b,nonzero rule] (175.7070,486.2910) -- (283.8730,486.2910) --
(283.8730,498.3750) -- (175.7070,498.3750) -- (175.7070,486.2910) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,486.2910) -- (175.7070,486.2910) --
(175.7070,498.3750) -- (283.8730,498.3750) -- (283.8730,486.2910) -- cycle;
\path[fill=c77797b,nonzero rule] (175.7070,406.0820) -- (283.8730,406.0820) --
(283.8730,418.1660) -- (175.7070,418.1660) -- (175.7070,406.0820) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,406.0820) -- (175.7070,406.0820) --
(175.7070,418.1660) -- (283.8730,418.1660) -- (283.8730,406.0820) --
cycle(220.2560,587.3940) -- (215.4649,587.3940) -- (215.4649,602.3210) --
(220.2560,602.3210) -- (220.2560,587.3940) -- cycle(215.4650,602.3210) --
(220.2560,587.3940)(215.5760,587.3940) --
(220.2560,602.3210)(243.8210,587.3940) -- (239.0309,587.3940) --
(239.0309,602.3210) -- (243.8210,602.3210) -- (243.8210,587.3940) --
cycle(239.0310,602.3210) -- (243.8210,587.3940)(239.1420,587.3940) --
(243.8210,602.3210)(217.5820,546.8440) -- (212.7910,546.8440) --
(212.7910,555.5315) -- (217.5820,555.5315) -- (217.5820,546.8440) --
cycle(212.7910,555.5310) -- (217.5820,546.8440)(212.9020,546.8440) --
(217.5820,555.5310)(246.3240,546.8440) -- (241.5340,546.8440) --
(241.5340,555.5315) -- (246.3240,555.5315) -- (246.3240,546.8440) --
cycle(241.5340,555.5310) -- (246.3240,546.8440)(241.6450,546.8440) --
(246.3240,555.5310)(217.5820,488.0800) -- (212.7910,488.0800) --
(212.7910,496.7670) -- (217.5820,496.7670) -- (217.5820,488.0800) --
cycle(212.7910,496.7670) -- (217.5820,488.0800)(212.9020,488.0800) --
(217.5820,496.7670)(246.3240,488.0800) -- (241.5340,488.0800) --
(241.5340,496.7670) -- (246.3240,496.7670) -- (246.3240,488.0800) --
cycle(241.5340,496.7670) -- (246.3240,488.0800)(241.6450,488.0800) --
(246.3240,496.7670)(217.5820,461.2320) -- (212.7910,461.2320) --
(212.7910,469.9190) -- (217.5820,469.9190) -- (217.5820,461.2320) --
cycle(212.7910,469.9190) -- (217.5820,461.2320)(212.9020,461.2320) --
(217.5820,469.9190)(246.3240,461.2320) -- (241.5340,461.2320) --
(241.5340,469.9190) -- (246.3240,469.9190) -- (246.3240,461.2320) --
cycle(241.5340,469.9190) -- (246.3240,461.2320)(241.6450,461.2320) --
(246.3240,469.9190)(217.5820,435.0540) -- (212.7910,435.0540) --
(212.7910,443.7420) -- (217.5820,443.7420) -- (217.5820,435.0540) --
cycle(212.7910,443.7420) -- (217.5820,435.0540)(212.9020,435.0540) --
(217.5820,443.7420)(246.3240,435.0540) -- (241.5340,435.0540) --
(241.5340,443.7420) -- (246.3240,443.7420) -- (246.3240,435.0540) --
cycle(241.5340,443.7420) -- (246.3240,435.0540)(241.6450,435.0540) --
(246.3240,443.7420)(217.5820,407.7510) -- (212.7910,407.7510) --
(212.7910,416.4390) -- (217.5820,416.4390) -- (217.5820,407.7510) --
cycle(212.7910,416.4390) -- (217.5820,407.7510)(212.9020,407.7510) --
(217.5820,416.4390)(246.3240,407.7510) -- (241.5340,407.7510) --
(241.5340,416.4390) -- (246.3240,416.4390) -- (246.3240,407.7510) --
cycle(241.5340,416.4390) -- (246.3240,407.7510)(241.6450,407.7510) --
(246.3240,416.4390)(217.5820,370.6620) -- (212.7910,370.6620) --
(212.7910,379.3490) -- (217.5820,379.3490) -- (217.5820,370.6620) --
cycle(212.7910,379.3490) -- (217.5820,370.6620)(212.9020,370.6620) --
(217.5820,379.3490)(246.3240,370.6620) -- (241.5340,370.6620) --
(241.5340,379.3490) -- (246.3240,379.3490) -- (246.3240,370.6620) --
cycle(241.5340,379.3490) -- (246.3240,370.6620)(241.6450,370.6620) --
(246.3240,379.3490)(217.5820,342.5840) -- (212.7910,342.5840) --
(212.7910,351.2720) -- (217.5820,351.2720) -- (217.5820,342.5840) --
cycle(212.7910,351.2720) -- (217.5820,342.5840)(212.9020,342.5840) --
(217.5820,351.2720)(246.3240,342.5840) -- (241.5340,342.5840) --
(241.5340,351.2720) -- (246.3240,351.2720) -- (246.3240,342.5840) --
cycle(241.5340,351.2720) -- (246.3240,342.5840)(241.6450,342.5840) --
(246.3240,351.2720)(229.4670,639.7080) -- (229.4670,306.5820);


\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,379.3490) {ISh};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,416.4390) {DPH2};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,443.7420) {DP22};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,469.9190) {DP21};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,496.7670) {DPH1};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,555.5310) {DP12};


\node[color=red!80!black, anchor=base west, yshift=0, xshift=-31.5] at (166.8500,626.0810) {OL};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,338.8890) {DStig};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,355.7310) {DSh};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,582.0560) {DP11};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,594.7750) {QPol};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,609.0010) {HPol};




\path[fill=c211e1f,nonzero rule] (229.4670,303.5640) .. controls
(228.9400,304.9840) and (228.0410,306.7460) .. (227.0900,307.8370) --
(229.4670,306.9770) -- (231.8440,307.8370) .. controls (230.8930,306.7460) and
(229.9930,304.9840) .. (229.4670,303.5640);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] 
(173.0060,322.0650)--(285.9290,322.0650)    %SAD Plane
(173.0060,626.0810) -- (285.9290,626.0810)  %Specimen Plane
(227.7460,632.2420) -- (231.4110,632.2420)
(227.7460,620.1720) -- (231.4110,620.1720)
%DSh and DStig
(165.9560,355.7310) -- (168.9040,355.7310) -- (168.9040,338.8890) -- (166.0970,338.8890)
(168.9040,347.1690) -- (171.9910,347.1690)
%HPol QPOL DP11
(165.9560,609.0010) -- (168.9040,609.0010) -- (168.9040,582.0560) -- (166.0970,582.0560)
(168.9040,594.7750) -- (171.9910,594.7750);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt,rounded corners=5pt, dashed, color=black]
(229.4670,626.0810) -- (275,620.0810) -- (275,585.9140) -- (202.8500,532.4150)--
(202.8500,472.0820) -- (256.1830,432.7480) -- (256.5170,391.9150) -- (229.4670,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt,rounded corners=5pt, dashed, color=red!80!black]
(229.4670,620.1720) -- (265,586.0810) -- (265,532.0820) -- (210.6840,471.9150) --
(210.6840,432.5820) -- (249.1840,391.5820) -- (270.8500,322.0650);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=black,rounded corners=5pt]
(250,626.0810) -- (250,585.9140) -- (219,532.4150)--
(180,472.0820) -- (260,432.7480) -- (275,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=red!80!black,rounded corners=5pt]
(229.4670,626.0810)-- (275,586.0810) -- (265,532.0820) --  (245,471.9150) -- 
(180,432.5820) -- (229.4670,322.0650);

%\path[cm={{1.0,0.0,0.0,-1.0,(147.9459,631.6819)}},fill=c211e1f,nonzero rule]
%(0.0000,0.0000) node[above right] (text6164) {OL pre ffp
%specimen plane bfp HPol QPol DP11 DP12
%TL11 TL12 HP1 TL21 TL22 HP2
%ADL SAD plane DPH1 DPH2 lSh DSh
%DStig DP21 DP22 OL post};




\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,632.2420) {ffp};
\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,620.1720) {bfp};


\end{scope}
\end{tikzpicture}


==> figures/chamber/chamber_old.tex <==
\pgfmathsetlength{\imagewidth}{\columnwidth}
\pgfmathsetlength{\imagescale}{\imagewidth/1024}

\begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
  \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0) {\includegraphics[width=\imagewidth]{figures/chamber/specimen_chamber.jpg}};
  \draw[ultra thick,white] (772,800) node [anchor=south west] {100\:mm} -- (1000,800);
  \node[yellow] at (850,100) [anchor=north] {ISO-K\:63 ports} ;
    \node[yellow] at (512,790) [anchor=north] {IGP port} ;
\end{tikzpicture}%


==> figures/cryo_resolution/tembench.tex <==
\pgfmathsetlength{\imagewidth}{.49\columnwidth}
\pgfmathsetlength{\imagescale}{\imagewidth/1024}
%\centering
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
      \tiny
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{../figures/tembench/140305_0024_calibrated_scaled}};
        \draw[ultra thick] (24,1000) node [anchor=south west] {50\:nm} -- (280,1000);
%        \node at (0,0) [anchor=north west] {(a)} ;
        \draw[thick] (371,263) rectangle (474,366);
        \draw[] (371,263) -- (512,0);
        \draw[] (371,366) -- (512,512);
        \draw[] (474,263) -- (1024,0);
        \draw[] (474,366) -- (1024,512);
        \draw[thick] (371,263) rectangle (474,366);

        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (512,0)
        {\includegraphics[width=.5\imagewidth]{../figures/tembench/140305_0024_calibrated_cut}};
        \draw[ultra thick] (536,488) node [anchor=south west] {10\:nm} -- (792,488);
        \draw[thick] (512,2) rectangle (1022,512);
      \end{tikzpicture}%
      \hfill
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
      \tiny
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{../figures/tembench/young_lorentz_plain}};
        \draw[thick,dashed,white] (512,512) circle (360);
        \node at (512,152) [anchor=south west, white] {1.1\:nm} ;
        \draw[ultra thick,white] (24,1000) node [anchor=south west, white] {1\:nm$^{\text{--1}}$} -- (424,1000);
 %       \node at (0,0) [anchor=north west, white] {(b)} ;
      \end{tikzpicture}%


==> figures/darkfield/darkfield_old.tex <==
%\subfloat[Alternative darkfield imaging mode \label{fig:darkfield}]{
%Matrix Optics darkfield paper.py


\definecolor{dGray}{gray}{0.7}
\definecolor{lGray}{gray}{0.9}
\definecolor{cb4b6b9}{RGB}{180,182,185}
\definecolor{c211e1f}{RGB}{33,30,31}
\definecolor{c77797b}{RGB}{119,121,123}
\def\y1{0.5}


\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-\y1, xscale=1.000000, inner sep=0pt, outer sep=0pt]
	\begin{scope}[cm={{2.062,0.0,0.0,-2.062,(-129.99548,1482.0161)}}]
	
%ol
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (280.9290,626.1980) .. controls					
	(280.9290,618.7370) and (252.3650,612.6880) .. (229.4670,612.6880) .. controls
	(206.5680,612.6880) and (178.0060,618.7370) .. (178.0060,626.1980) .. controls
	(178.0060,633.6590) and (206.5680,639.7080) .. (229.4670,639.7080) .. controls
	(252.3650,639.7080) and (280.9290,633.6590) .. (280.9290,626.1980);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line width=0.400pt] 
(280.9290,626.1980) .. controls (280.9290,618.7370) and
(252.3650,612.6880) .. (229.4670,612.6880) .. controls (206.5680,612.6880) and
(178.0060,618.7370) .. (178.0060,626.1980) .. controls (178.0060,633.6590) and
(206.5680,639.7080) .. (229.4670,639.7080) .. controls (252.3650,639.7080) and
(280.9290,633.6590) .. (280.9290,626.1980) -- cycle;

%tl11
\path[fill=cb4b6b9,nonzero rule,color=lightgray] (283.7750,586.0280) .. controls
(283.7750,582.2590) and (248.4730,579.2040) .. (229.5980,579.2040) .. controls
(210.7230,579.2040) and (175.4200,582.2590) .. (175.4200,586.0280) .. controls
(175.4200,589.7960) and (210.7230,592.8500) .. (229.5980,592.8500) .. controls
(248.4730,592.8500) and (283.7750,589.7960) .. (283.7750,586.0280);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.7750,586.0280) .. controls (283.7750,582.2590) and
(248.4730,579.2040) .. (229.5980,579.2040) .. controls (210.7230,579.2040) and
(175.4200,582.2590) .. (175.4200,586.0280) .. controls (175.4200,589.7960) and
(210.7230,592.8500) .. (229.5980,592.8500) .. controls (248.4730,592.8500) and
(283.7750,589.7960) .. (283.7750,586.0280) -- cycle;

%tl12
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.0290,532.5260) .. controls
(283.0290,528.8980) and (248.7270,525.9580) .. (229.8510,525.9580) .. controls
(210.9750,525.9580) and (175.6740,528.8980) .. (175.6740,532.5260) .. controls
(175.6740,536.1530) and (210.9750,539.0930) .. (229.8510,539.0930) .. controls
(248.7270,539.0930) and (283.0290,536.1530) .. (283.0290,532.5260);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.0290,532.5260) .. controls (283.0290,528.8980) and
(248.7270,525.9580) .. (229.8510,525.9580) .. controls (210.9750,525.9580) and
(175.6740,528.8980) .. (175.6740,532.5260) .. controls (175.6740,536.1530) and
(210.9750,539.0930) .. (229.8510,539.0930) .. controls (248.7270,539.0930) and
(283.0290,536.1530) .. (283.0290,532.5260) -- cycle;

%Tl21
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,472.3160) .. controls
(283.9060,468.6220) and (248.6320,465.6260) .. (229.7890,465.6260) .. controls
(210.9470,465.6260) and (175.6720,468.6220) .. (175.6720,472.3160) .. controls
(175.6720,476.0110) and (210.9470,479.0060) .. (229.7890,479.0060) .. controls
(248.6320,479.0060) and (283.9060,476.0110) .. (283.9060,472.3160);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,472.3160) .. controls (283.9060,468.6220) and
(248.6320,465.6260) .. (229.7890,465.6260) .. controls (210.9470,465.6260) and
(175.6720,468.6220) .. (175.6720,472.3160) .. controls (175.6720,476.0110) and
(210.9470,479.0060) .. (229.7890,479.0060) .. controls (248.6320,479.0060) and
(283.9060,476.0110) .. (283.9060,472.3160) -- cycle;

%Tl22
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,432.8440) .. controls
(283.9060,429.1500) and (248.6320,426.1550) .. (229.7890,426.1550) .. controls
(210.9470,426.1550) and (175.6720,429.1500) .. (175.6720,432.8440) .. controls
(175.6720,436.5390) and (210.9470,439.5350) .. (229.7890,439.5350) .. controls
(248.6320,439.5350) and (283.9060,436.5390) .. (283.9060,432.8440);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,432.8440) .. controls (283.9060,429.1500) and
(248.6320,426.1550) .. (229.7890,426.1550) .. controls (210.9470,426.1550) and
(175.6720,429.1500) .. (175.6720,432.8440) .. controls (175.6720,436.5390) and
(210.9470,439.5350) .. (229.7890,439.5350) .. controls (248.6320,439.5350) and
(283.9060,436.5390) .. (283.9060,432.8440) -- cycle;

%adl
\path[fill=cb4b6b9,nonzero rule,color=lightgray] (283.9060,391.8650) .. controls
(283.9060,388.1700) and (248.6320,385.1750) .. (229.7890,385.1750) .. controls
(210.9470,385.1750) and (175.6720,388.1700) .. (175.6720,391.8650) .. controls
(175.6720,395.5590) and (210.9470,398.5550) .. (229.7890,398.5550) .. controls
(248.6320,398.5550) and (283.9060,395.5590) .. (283.9060,391.8650);


\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,391.8650) {ADL};
\node[color=red!80!black, anchor=base west, yshift=6*\y1, xshift=5] at (286.9230,404.0820) {HP2};
\node[color=red!80!black, anchor=base west, yshift=8*\y1, xshift=5] at (286.9230,483.2910) {HP1};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,432.8440) {TL22};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,472.3160) {Tl21};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,532.5260) {TL12};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,586.0280) {TL11};

\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,322.0650) {SAD plane};
\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,626.0810) {specimen plane};


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,391.8650) .. controls (283.9060,388.1700) and
(248.6320,385.1750) .. (229.7890,385.1750) .. controls (210.9470,385.1750) and
(175.6720,388.1700) .. (175.6720,391.8650) .. controls (175.6720,395.5590) and
(210.9470,398.5550) .. (229.7890,398.5550) .. controls (248.6320,398.5550) and
(283.9060,395.5590) .. (283.9060,391.8650) -- cycle;

%HP1
\path[fill=c77797b,nonzero rule,pattern=north west lines,pattern color=lightgray] (175.7070,486.2910) -- (283.8730,486.2910) --
(283.8730,498.3750) -- (175.7070,498.3750) -- (175.7070,486.2910) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,486.2910) -- (175.7070,486.2910) --
(175.7070,498.3750) -- (283.8730,498.3750) -- (283.8730,486.2910) -- cycle;
%HP2
\path[fill=c77797b,nonzero rule,pattern=north west lines,pattern color=lightgray] (175.7070,406.0820) -- (283.8730,406.0820) --
(283.8730,418.1660) -- (175.7070,418.1660) -- (175.7070,406.0820) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,406.0820) -- (175.7070,406.0820) --
(175.7070,418.1660) -- (283.8730,418.1660) -- (283.8730,406.0820) --
cycle(220.2560,587.3940) -- (215.4649,587.3940) -- (215.4649,602.3210) --
(220.2560,602.3210) -- (220.2560,587.3940) -- cycle(215.4650,602.3210) --
(220.2560,587.3940)(215.5760,587.3940) --
(220.2560,602.3210)(243.8210,587.3940) -- (239.0309,587.3940) --
(239.0309,602.3210) -- (243.8210,602.3210) -- (243.8210,587.3940) --
cycle(239.0310,602.3210) -- (243.8210,587.3940)(239.1420,587.3940) --
(243.8210,602.3210)(217.5820,546.8440) -- (212.7910,546.8440) --
(212.7910,555.5315) -- (217.5820,555.5315) -- (217.5820,546.8440) --
cycle(212.7910,555.5310) -- (217.5820,546.8440)(212.9020,546.8440) --
(217.5820,555.5310)(246.3240,546.8440) -- (241.5340,546.8440) --
(241.5340,555.5315) -- (246.3240,555.5315) -- (246.3240,546.8440) --
cycle(241.5340,555.5310) -- (246.3240,546.8440)(241.6450,546.8440) --
(246.3240,555.5310)(217.5820,488.0800) -- (212.7910,488.0800) --
(212.7910,496.7670) -- (217.5820,496.7670) -- (217.5820,488.0800) --
cycle(212.7910,496.7670) -- (217.5820,488.0800)(212.9020,488.0800) --
(217.5820,496.7670)(246.3240,488.0800) -- (241.5340,488.0800) --
(241.5340,496.7670) -- (246.3240,496.7670) -- (246.3240,488.0800) --
cycle(241.5340,496.7670) -- (246.3240,488.0800)(241.6450,488.0800) --
(246.3240,496.7670)(217.5820,461.2320) -- (212.7910,461.2320) --
(212.7910,469.9190) -- (217.5820,469.9190) -- (217.5820,461.2320) --
cycle(212.7910,469.9190) -- (217.5820,461.2320)(212.9020,461.2320) --
(217.5820,469.9190)(246.3240,461.2320) -- (241.5340,461.2320) --
(241.5340,469.9190) -- (246.3240,469.9190) -- (246.3240,461.2320) --
cycle(241.5340,469.9190) -- (246.3240,461.2320)(241.6450,461.2320) --
(246.3240,469.9190)(217.5820,435.0540) -- (212.7910,435.0540) --
(212.7910,443.7420) -- (217.5820,443.7420) -- (217.5820,435.0540) --
cycle(212.7910,443.7420) -- (217.5820,435.0540)(212.9020,435.0540) --
(217.5820,443.7420)(246.3240,435.0540) -- (241.5340,435.0540) --
(241.5340,443.7420) -- (246.3240,443.7420) -- (246.3240,435.0540) --
cycle(241.5340,443.7420) -- (246.3240,435.0540)(241.6450,435.0540) --
(246.3240,443.7420)(217.5820,407.7510) -- (212.7910,407.7510) --
(212.7910,416.4390) -- (217.5820,416.4390) -- (217.5820,407.7510) --
cycle(212.7910,416.4390) -- (217.5820,407.7510)(212.9020,407.7510) --
(217.5820,416.4390)(246.3240,407.7510) -- (241.5340,407.7510) --
(241.5340,416.4390) -- (246.3240,416.4390) -- (246.3240,407.7510) --
cycle(241.5340,416.4390) -- (246.3240,407.7510)(241.6450,407.7510) --
(246.3240,416.4390)(217.5820,370.6620) -- (212.7910,370.6620) --
(212.7910,379.3490) -- (217.5820,379.3490) -- (217.5820,370.6620) --
cycle(212.7910,379.3490) -- (217.5820,370.6620)(212.9020,370.6620) --
(217.5820,379.3490)(246.3240,370.6620) -- (241.5340,370.6620) --
(241.5340,379.3490) -- (246.3240,379.3490) -- (246.3240,370.6620) --
cycle(241.5340,379.3490) -- (246.3240,370.6620)(241.6450,370.6620) --
(246.3240,379.3490)(217.5820,342.5840) -- (212.7910,342.5840) --
(212.7910,351.2720) -- (217.5820,351.2720) -- (217.5820,342.5840) --
cycle(212.7910,351.2720) -- (217.5820,342.5840)(212.9020,342.5840) --
(217.5820,351.2720)(246.3240,342.5840) -- (241.5340,342.5840) --
(241.5340,351.2720) -- (246.3240,351.2720) -- (246.3240,342.5840) --
cycle(241.5340,351.2720) -- (246.3240,342.5840)(241.6450,342.5840) --
(246.3240,351.2720)(229.4670,639.7080) -- (229.4670,306.5820);


\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,379.3490) {ISh};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,416.4390) {DPH2};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,443.7420) {DP22};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,469.9190) {DP21};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,496.7670) {DPH1};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,555.5310) {DP12};


\node[color=red!80!black, anchor=base west, yshift=0, xshift=-31.5] at (166.8500,626.0810) {OL};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,338.8890) {DStig};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,355.7310) {DSh};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,582.0560) {DP11};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,594.7750) {QPol};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,609.0010) {HPol};




\path[fill=c211e1f,nonzero rule] (229.4670,303.5640) .. controls
(228.9400,304.9840) and (228.0410,306.7460) .. (227.0900,307.8370) --
(229.4670,306.9770) -- (231.8440,307.8370) .. controls (230.8930,306.7460) and
(229.9930,304.9840) .. (229.4670,303.5640);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] 
(173.0060,322.0650)--(285.9290,322.0650)    %SAD Plane
(173.0060,626.0810) -- (285.9290,626.0810)  %Specimen Plane

%bfp ffp
%(227.7460,632.2420) -- (231.4110,632.2420)
%(227.7460,620.1720) -- (231.4110,620.1720)
%DSh and DStig
(165.9560,355.7310) -- (168.9040,355.7310) -- (168.9040,338.8890) -- (166.0970,338.8890)
(168.9040,347.1690) -- (171.9910,347.1690)
%HPol QPOL DP11
(165.9560,609.0010) -- (168.9040,609.0010) -- (168.9040,582.0560) -- (166.0970,582.0560)
(168.9040,594.7750) -- (171.9910,594.7750);


%\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
%width=0.400pt,rounded corners=5pt, dashed, color=black]
%(229.4670,626.0810) -- (275,620.0810) -- (275,585.9140) -- (202.8500,532.4150)--
%(202.8500,472.0820) -- (256.1830,432.7480) -- (256.5170,391.9150) -- (229.4670,322.0650);

%\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
%width=0.400pt,rounded corners=5pt, dashed, color=red!80!black]
%(229.4670,620.1720) -- (265,586.0810) -- (265,532.0820) -- (210.6840,471.9150) --
%(210.6840,432.5820) -- (249.1840,391.5820) -- (270.8500,322.0650);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=black,rounded corners=5pt]
(249.4670,626.0810) -- (249.4670,585.9140) -- (180,390) -- (229.4670,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=red!80!black,rounded corners=5pt]
(229.4670,626.0810)-- (255,586.0810) -- (235,390) -- (215,322.0650)
(249.4670,626.0810)-- (275,586.0810) -- (182,390) -- (215,322.0650);


%\path[cm={{1.0,0.0,0.0,-1.0,(147.9459,631.6819)}},fill=c211e1f,nonzero rule]
%(0.0000,0.0000) node[above right] (text6164) {OL pre ffp
%specimen plane bfp HPol QPol DP11 DP12
%TL11 TL12 HP1 TL21 TL22 HP2
%ADL SAD plane DPH1 DPH2 lSh DSh
%DStig DP21 DP22 OL post};




%\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,632.2420) {ffp};
%\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,620.1720) {bfp};


\end{scope}
\end{tikzpicture}



==> figures/holo/holo.tex <==
\begin{tikzpicture}[xscale=0.7,yscale=0.5]
%\draw [help lines] (-5,-5) grid (5,5);




\def\t{0.5} 
\def\s{0.25}
\def\nub{5} % anz. der Strahlen


%undiffracted beam

\foreach \x in {1,3,5,...,\nub}    
	\draw [black, thick,rounded corners=8pt](0,6) -- (\x/2-1/2-\nub/4+1/4,3) -- (\x/2-1/2-\nub/4+1/4,0) -- (\x/2-1/2-\nub/4+1/4,-2) -- (-\x+1+\nub/2-1/2,-9) -- (-\x*1.25+\nub/2+1.25,-12);

%virtual beam 1

\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (1.35,-4.325) -- (0,0);
\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (-1.35,-4.325) -- (0,0);

\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (1.35,-4.325) -- (2.5,-12);
\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (1.35,-4.325) -- (-.5,-12);

\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (-1.35,-4.325) -- (-2.5,-12);
\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (-1.35,-4.325) -- (.5,-12);
\node[color=red!80!black] at (-1.65,-4.325+0.6) {$-\boldsymbol{\frac{q_c}{2}}$};
\node[color=red!80!black] at (1.6,-4.325+0.6) {$+\boldsymbol{\frac{q_c}{2}}$};
\filldraw[color=red!80!black] (-1.35-0.04,-4.325) arc (180:-180:0.0253/0.7 and 0.056); 
\filldraw[color=red!80!black] (1.35-0.04,-4.325) arc (180:-180:0.0253/0.7 and 0.056); 

%virtual beam 2
%\foreach \x in {1,5,...,\nub}    
%	\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (\x/1.5-1/2-\nub/4-1/4,-4.325) -- (\x-1-\nub/2+1/2,-9) -- (-2.5,-12);
%\foreach \x in {1,5,...,\nub}    
%	\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (\x/1.5-1/2-\nub/4-1/4,-4.325) -- (-\x/4+\nub/2-1.75,-12);


%diffracted beam  
\draw [red!80!black,opacity=.7, thick,rounded corners=8pt] (0.5,0)  -- (0.25,-2) -- (-1.1,-9) -- (-1,-12);
\draw [red!80!black,opacity=.7, thick,rounded corners=8pt] (0.5,0)  -- (0.75,-2) -- (-0.95,-9) -- (-1,-12);


%image and ref wave
%image
\fill [red!80!black,opacity=.3, thick,rounded corners=5pt] (0 ,0)  -- (0,-12.2) -- (-2.53,-12.2) -- (-2,-9) -- (1,-2) -- (1,0);
%ref
\fill [black,opacity=.3, thick,rounded corners=5pt] (0 ,0)  -- (0,-12.2) -- (2.53,-12.2) -- (2,-9) -- (-1,-2) -- (-1,0);


% annotation B
%\filldraw [fill=white ,draw=white] (3.3,{0.0+1}) circle (0.24) [path picture={ \node at (path picture bounding box.center) {$\color{red}\mathrm{\boldsymbol{B}}$};} ];
%\filldraw [fill=white ,draw=white] (3.3,{0.0-1}) circle (0.24) [path picture={ \node at (path picture bounding box.center) {$\color{red}\mathrm{\boldsymbol{B}}$};} ];


% biprism
\filldraw[draw=black, line width=0.25 ,fill=red!80!black] (-.18,-9)  arc (180:-180:0.125/0.7 and 0.25);
\filldraw[draw=black, line width=0.25 ,fill=red!80!black] (-3,-8.5) -- (-3,-9.5)--(-3.05,-9.5)--(-3.05,-8.5)--(-3,-8.5);
\filldraw[draw=black, line width=0.25 ,fill=red!80!black] (3,-8.5) -- (3,-9.5)--(3.05,-9.5)--(3.05,-8.5)--(3,-8.5);
\draw [black, line width=0.25] (3.05,-9.25)  -- (3.25,-9.25)-- (3.25,-9.75);
\draw [black, line width=0.25] (3.1,-9.75) -- (3.4,-9.75);
\draw [black, line width=0.25] (3.15,-9.85) -- (3.35,-9.85);
\draw [black, line width=0.25] (3.2,-9.95) -- (3.3,-9.95);

\draw [black, line width=0.25] (-3.05,-9.25)  -- (-3.25,-9.25)-- (-3.25,-9.75);
\draw [black, line width=0.25] (-3.1,-9.75) -- (-3.4,-9.75);
\draw [black, line width=0.25] (-3.15,-9.85) -- (-3.35,-9.85);
\draw [black, line width=0.25] (-3.2,-9.95) -- (-3.3,-9.95);


\draw [black, thick] (0.1,-9)  -- (-0.1,-9);
\draw [black, thick] (0,-9.14)  -- (0,-8.86);


%specimen, image and hologramm	

\filldraw[draw=black, line width=0.25 ,fill=red!80!black,rounded corners=0.3pt] (-0.025,0)--(2,0)--(2,0.2) --(-0.025,0.2)--(-0.025,0)--(2,0);
\filldraw[draw=black, line width=0.25 ,fill=red!80!black,rounded corners=0.3pt] (0.55,-12)--(-2.55,-12)--(-2.55,-12.2) --(0.55,-12.2)--(0.55,-12)--(-2.55,-12);
\def\anz{20}
\foreach \x in {0,1,2,...,\anz}    
	\draw [black,opacity=.7,rounded corners=8pt] (-0.5+\x/\anz,-12.2) -- (-0.5+\x/\anz,-12);



%lenses
%conderser
\fill[gray,opacity=.5] (-2,2.9)  arc (180:-180:2 and 0.2);
%main imaging lens
\fill[gray,opacity=.5] (-4,-1.9)  arc (180:-180:4 and 0.2);

%specimen plane

\draw [black,opacity=.7, thick,dashed] (-4,0) -- (4,0);
\node[color=red!80!black, anchor=base west] at (3,0.25) {specimen plane};

%backfocal plane

\draw [black,opacity=.7, thick,dashed] (-4,-4.325) -- (4,-4.325);
\node[color=red!80!black, anchor=base west] at (3,-4.325+0.25) {back focal plane};


%image plane

\draw [black,opacity=.7, thick,dashed] (-4,-12.2) -- (4,-12.2);
\node[color=red!80!black, anchor=base west] at (3,-12.2+0.25) {image plane};

%annotaions

\node[color=red!80!black, anchor=base west] at (-5.5,-9.125) {biprism};
\node[color=red!80!black, anchor=base west] at (-5.5,-2+0.5) {main imaging lens};
\node[color=red!80!black, anchor=base west] at (-5.5,3+0.1) {condenser system};
\node[color=red!80!black] at (0,-12-0.7) {hologramm};


\draw [<->] (1,-8.55) -- (3,-8.55) [-stealth, line width=0.25pt, black];
\draw [<->] (2,-8.55) -- (0,-8.55) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (1.1,-9.15) {$\mathrm{d_{bp}}$};


\draw [<->] (0.25,-11.8) -- (0.5,-11.8) [-stealth, line width=0.25pt, black];
\draw [<->] (0.25,-11.8) -- (-0.5,-11.8) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-0.11,-11.55) {$\mathrm{w_{hol}}$};


\draw [<->] (-2.75,-3) -- (-2.75,-4.325) [-stealth, line width=0.25pt, black];
\draw [<->] (-2.75,-4) -- (-2.75,-1.9) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-2.8,-3.35) {$\mathrm{f}$};

\draw [<->] (-2.75,-5) -- (-2.75,-9) [-stealth, line width=0.25pt, black];
\draw [<->] (-2.75,-6) -- (-2.75,-4.325) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-2.8,-6.8) {$\mathrm{a}$};

\draw [<->] (-2.75,-10) -- (-2.75,-12.2) [-stealth, line width=0.25pt, black];
\draw [<->] (-2.75,-11) -- (-2.75,-9) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-2.8,-10.8) {$\mathrm{b}$};


\draw[black] (-1.77,-7.0275)  arc (78:50:1 and 2);
\node[black, anchor=base west] at (-1.7,-7) {$\gamma$};



\draw[black] (0.265,-0.8)  arc (-58:-122:0.5 and 1);
\node[black, anchor=base west] at (-0.5,-1.52) {$\beta$};


\end{tikzpicture}


==> figures/raypaths/raypaths.tex <==
\subfloat[Standard imaging mode with excited objective lens \label{fig:Image mode ol on}]{
%Matrix Optics Diff non OL.py

\begin{tikzpicture}[yscale=0.5, xscale=0.75]



\def\s{0.7}

\def\nub{5}

%\draw [help lines] (-5,3) grid (5,-5);

\def\xa{1}
\def\xb{0}
\def\xc{-1.5}
\def\xd{-6.5}
\def\xe{-8.5}


% 0 beam

\draw [black,opacity=.7, thick,rounded corners=8pt ] (0,\xa) -- (0,\xb) -- (0,\xc) -- (0,\xd) -- (0,\xe);
\draw [black,opacity=.7, thick,rounded corners=8pt ] (0.5,\xa) -- (0.5,\xb) -- (0.5,\xc) -- (-2,\xd) -- (1,\xe);



%+1 beam 

\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0,\xb) -- (0.40192378864668404,\xc) -- (-0.26794919243112275,\xd) -- (0,\xe);
\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0.5,\xb) -- (0.90192378864668399,\xc) -- (-2.2679491924311224,\xd) -- (1.0,\xe);


%+2 beam 

\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0,\xb) -- (0.8660254037844386,\xc) -- (-0.57735026918962573,\xd) -- (0.0,\xe);
\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0.5,\xb) -- (1.3660254037844386,\xc) -- (-2.5773502691896262,\xd) -- (1.0,\xe);


%objective lens

\fill[gray,opacity=.5] (-3,\xc+0.05)  arc (180:-180:3 and 0.3);

	% Schrift

\node[color=red!80!black, anchor=base west] at (-4.25,\xc+0.5+0.05) {objective lens} ;


% transfer system

\fill[gray,opacity=.5] (-5,\xd+0.5) -- (5, \xd+0.5) -- (5, \xd-0.5) -- (-5, \xd-0.5) -- (-5, \xd+0.5)   ;

	% Schrift

\node[color=red!80!black, anchor=base west] at (0.5,\xd+0.7) {transfer system} ;


%Specimen 
\fill[gray,opacity=.7] (-2,\xb+0.05)   rectangle (2,\xb-0.05) ;
\draw [black,opacity=.7, thick,dotted] (-5,0) -- (5,0);
	% Schrift
\node[color=red!80!black, anchor=base west] at (0.5,\xb+0.2) {specimen plane} ;

%image Plane

\draw [black,opacity=.7, thick,dotted] (-5,\xe) -- (5,\xe);
	% Schrift
\node[color=red!80!black, anchor=base west] at (-4.25,\xe+0.2) {image plane} ;

\end{tikzpicture}

}\hfill{}\subfloat[Imaging mode without objective lens \label{fig:Image mode ol off}]{
%werte aus Matrix Optics Diff non OL.py

\begin{tikzpicture}[yscale=0.5, xscale=0.75]



\def\s{0.7}

\def\nub{5}

%\draw [help lines] (-5,3) grid (5,-5);

\def\xa{1}
\def\xb{0}
\def\xc{-1.5}
\def\xd{-6.5}
\def\xe{-8.5}


% 0 beam

\draw [black,opacity=.7, thick,rounded corners=8pt ] (0,\xa) -- (0,\xb) -- (0,\xc) -- (0,\xd) -- (0,\xe);
\draw [black,opacity=.7, thick,rounded corners=8pt ] (0.5,\xa) -- (0.5,\xb) -- (0.5,\xc) -- (0.5,\xd) -- (-0.15385118347064208,\xe);
 

%+1 beam 

\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0,\xb) -- (0.40192378864668404,\xc) -- (1.7416697508022976,\xd) -- (0,\xe);
\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0.5,\xb) -- (0.90192378864668399,\xc) -- (2.2416697508022976,\xd) -- (-0.1538687033602999,\xe);


%+2 beam 

\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0,\xb) -- (0.8660254037844386,\xc) -- (3.7527767497325675,\xd) -- (0,\xe);
\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0.5,\xb) -- (1.3660254037844386,\xc) -- (4.2527767497325675,\xd) -- (-0.1538889335863205,\xe);


%objective lens

\fill[gray,opacity=.15] (-3,\xc+0.05)  arc (180:-180:3 and 0.3);

	% Schrift

\node[color=red!80!black, anchor=base west] at (-4.25,\xc+0.5+0.05) {objective lens} ;

% transfer system

\fill[gray,opacity=.5] (-5,\xd+0.5) -- (5, \xd+0.5) -- (5, \xd-0.5) -- (-5, \xd-0.5) -- (-5, \xd+0.5)   ;

	% Schrift

\node[color=red!80!black, anchor=base west] at (-4.25,\xd+0.7) {transfer system} ;



%Specimen 
\fill[gray,opacity=.7] (-2,\xb+0.05)   rectangle (2,\xb-0.05) ;
\draw [black,opacity=.7, thick,dotted] (-5,0) -- (5,0);
	% Schrift
\node[color=red!80!black, anchor=base west] at (0.5,\xb+0.2) {specimen plane} ;

%Image Plane

\draw [black,opacity=.7, thick,dotted] (-5,\xe) -- (5,\xe);
	% Schrift
\node[color=red!80!black, anchor=base west] at (-4.25,\xe+0.2) {image plane} ;
\end{tikzpicture}

}



==> for arxiv 2/figures/calibtemp/calibtemp_2.tex <==
%\pgfmathsetlength{\imagewidth}{.24\textwidth}
\pgfmathsetlength{\imagewidth}{.49\columnwidth}
\pgfmathsetlength{\imagescale}{\imagewidth/1024}

      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{figures/calibtemp/130K_2}};
        \draw[ultra thick] (24,1000) node [anchor=south west] {2\:nm$^{\text{--1}}$} -- (250,1000);
        \node at (0,0) [anchor=north west] {(a)} ;
        \node at (1024,0) [anchor=north east] {130\:K} ;
      \end{tikzpicture}%
      \hfill
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{figures/calibtemp/120K_2}};
        \draw[] (768,303) node [anchor=south east] {$q_{\frac{2}{3}}$} circle (20);
        \draw[] (724,402) node [anchor=south east] {$q_{\frac{1}{3}}$} circle (20);
        \node at (0,0) [anchor=north west] {(b)} ;
        \node at (1024,0) [anchor=north east] {120\:K} ;
      \end{tikzpicture}%
      %% \hfill
      %% \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      %% \sffamily
      %%   \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
      %%   {\includegraphics[width=\imagewidth]{figures/calibtemp/90K_2}};
      %%   \draw[] (768,303) node [anchor=south east] {$q_{\frac{2}{3}}$} circle (20);
      %%   \draw[] (724,402) node [anchor=south east] {$q_{\frac{1}{3}}$} circle (20);
      %%   \node at (0,0) [anchor=north west] {(c)} ;
      %%   \node at (1024,0) [anchor=north east] {90\:K} ;
      %% \end{tikzpicture}%
      %% \hfill
      %% \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      %% \sffamily
      %%   \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
      %%   {\includegraphics[width=\imagewidth]{figures/calibtemp/80K_2}};
      %%   \draw[] (768,303) node [anchor=south east] {$q_{\frac{2}{3}(1-\delta)}$} circle (20);
      %%   \draw[] (724,402) node [anchor=south east] {$q_{\frac{1}{3}(1-\delta)}$} circle (20);
      %%   \node at (0,0) [anchor=north west] {(d)} ;
      %%   \node at (1024,0) [anchor=north east] {80\:K} ;
      %% \end{tikzpicture}%


==> for arxiv 2/figures/cetcor/cetcor.tex <==
\definecolor{cb4b6b9}{RGB}{180,182,185}
\definecolor{c211e1f}{RGB}{33,30,31}
\definecolor{c77797b}{RGB}{119,121,123}
\def\y1{0.5}
\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-\y1, xscale=0.8, inner sep=0pt, outer sep=0pt]
	\begin{scope}[cm={{2.062,0.0,0.0,-2.062,(-129.99548,1482.0161)}}]
	
%ol
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (280.9290,626.1980) .. controls					
	(280.9290,618.7370) and (252.3650,612.6880) .. (229.4670,612.6880) .. controls
	(206.5680,612.6880) and (178.0060,618.7370) .. (178.0060,626.1980) .. controls
	(178.0060,633.6590) and (206.5680,639.7080) .. (229.4670,639.7080) .. controls
	(252.3650,639.7080) and (280.9290,633.6590) .. (280.9290,626.1980);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line width=0.400pt] 
(280.9290,626.1980) .. controls (280.9290,618.7370) and
(252.3650,612.6880) .. (229.4670,612.6880) .. controls (206.5680,612.6880) and
(178.0060,618.7370) .. (178.0060,626.1980) .. controls (178.0060,633.6590) and
(206.5680,639.7080) .. (229.4670,639.7080) .. controls (252.3650,639.7080) and
(280.9290,633.6590) .. (280.9290,626.1980) -- cycle;


\path[fill=cb4b6b9,nonzero rule] (283.7750,586.0280) .. controls
(283.7750,582.2590) and (248.4730,579.2040) .. (229.5980,579.2040) .. controls
(210.7230,579.2040) and (175.4200,582.2590) .. (175.4200,586.0280) .. controls
(175.4200,589.7960) and (210.7230,592.8500) .. (229.5980,592.8500) .. controls
(248.4730,592.8500) and (283.7750,589.7960) .. (283.7750,586.0280);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.7750,586.0280) .. controls (283.7750,582.2590) and
(248.4730,579.2040) .. (229.5980,579.2040) .. controls (210.7230,579.2040) and
(175.4200,582.2590) .. (175.4200,586.0280) .. controls (175.4200,589.7960) and
(210.7230,592.8500) .. (229.5980,592.8500) .. controls (248.4730,592.8500) and
(283.7750,589.7960) .. (283.7750,586.0280) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.0290,532.5260) .. controls
(283.0290,528.8980) and (248.7270,525.9580) .. (229.8510,525.9580) .. controls
(210.9750,525.9580) and (175.6740,528.8980) .. (175.6740,532.5260) .. controls
(175.6740,536.1530) and (210.9750,539.0930) .. (229.8510,539.0930) .. controls
(248.7270,539.0930) and (283.0290,536.1530) .. (283.0290,532.5260);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.0290,532.5260) .. controls (283.0290,528.8980) and
(248.7270,525.9580) .. (229.8510,525.9580) .. controls (210.9750,525.9580) and
(175.6740,528.8980) .. (175.6740,532.5260) .. controls (175.6740,536.1530) and
(210.9750,539.0930) .. (229.8510,539.0930) .. controls (248.7270,539.0930) and
(283.0290,536.1530) .. (283.0290,532.5260) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.9060,472.3160) .. controls
(283.9060,468.6220) and (248.6320,465.6260) .. (229.7890,465.6260) .. controls
(210.9470,465.6260) and (175.6720,468.6220) .. (175.6720,472.3160) .. controls
(175.6720,476.0110) and (210.9470,479.0060) .. (229.7890,479.0060) .. controls
(248.6320,479.0060) and (283.9060,476.0110) .. (283.9060,472.3160);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,472.3160) .. controls (283.9060,468.6220) and
(248.6320,465.6260) .. (229.7890,465.6260) .. controls (210.9470,465.6260) and
(175.6720,468.6220) .. (175.6720,472.3160) .. controls (175.6720,476.0110) and
(210.9470,479.0060) .. (229.7890,479.0060) .. controls (248.6320,479.0060) and
(283.9060,476.0110) .. (283.9060,472.3160) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.9060,432.8440) .. controls
(283.9060,429.1500) and (248.6320,426.1550) .. (229.7890,426.1550) .. controls
(210.9470,426.1550) and (175.6720,429.1500) .. (175.6720,432.8440) .. controls
(175.6720,436.5390) and (210.9470,439.5350) .. (229.7890,439.5350) .. controls
(248.6320,439.5350) and (283.9060,436.5390) .. (283.9060,432.8440);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,432.8440) .. controls (283.9060,429.1500) and
(248.6320,426.1550) .. (229.7890,426.1550) .. controls (210.9470,426.1550) and
(175.6720,429.1500) .. (175.6720,432.8440) .. controls (175.6720,436.5390) and
(210.9470,439.5350) .. (229.7890,439.5350) .. controls (248.6320,439.5350) and
(283.9060,436.5390) .. (283.9060,432.8440) -- cycle;
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,391.8650) .. controls
(283.9060,388.1700) and (248.6320,385.1750) .. (229.7890,385.1750) .. controls
(210.9470,385.1750) and (175.6720,388.1700) .. (175.6720,391.8650) .. controls
(175.6720,395.5590) and (210.9470,398.5550) .. (229.7890,398.5550) .. controls
(248.6320,398.5550) and (283.9060,395.5590) .. (283.9060,391.8650);


\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,391.8650) {ADL};
\node[color=red!80!black, anchor=base west, yshift=6*\y1, xshift=5] at (286.9230,406.0820) {HP2};
\node[color=red!80!black, anchor=base west, yshift=8*\y1, xshift=5] at (286.9230,486.2910) {HP1};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,432.8440) {TL22};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,472.3160) {Tl21};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,532.5260) {TL12};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,586.0280) {TL11};

\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,322.0650) {SA plane};
\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,626.0810) {specimen};

%\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (260.9230,326) {SA plane};
%\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (260,630) {specimen plane};


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,391.8650) .. controls (283.9060,388.1700) and
(248.6320,385.1750) .. (229.7890,385.1750) .. controls (210.9470,385.1750) and
(175.6720,388.1700) .. (175.6720,391.8650) .. controls (175.6720,395.5590) and
(210.9470,398.5550) .. (229.7890,398.5550) .. controls (248.6320,398.5550) and
(283.9060,395.5590) .. (283.9060,391.8650) -- cycle;
\path[fill=c77797b,nonzero rule] (175.7070,486.2910) -- (283.8730,486.2910) --
(283.8730,498.3750) -- (175.7070,498.3750) -- (175.7070,486.2910) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,486.2910) -- (175.7070,486.2910) --
(175.7070,498.3750) -- (283.8730,498.3750) -- (283.8730,486.2910) -- cycle;
\path[fill=c77797b,nonzero rule] (175.7070,406.0820) -- (283.8730,406.0820) --
(283.8730,418.1660) -- (175.7070,418.1660) -- (175.7070,406.0820) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,406.0820) -- (175.7070,406.0820) --
(175.7070,418.1660) -- (283.8730,418.1660) -- (283.8730,406.0820) --
cycle(220.2560,587.3940) -- (215.4649,587.3940) -- (215.4649,602.3210) --
(220.2560,602.3210) -- (220.2560,587.3940) -- cycle(215.4650,602.3210) --
(220.2560,587.3940)(215.5760,587.3940) --
(220.2560,602.3210)(243.8210,587.3940) -- (239.0309,587.3940) --
(239.0309,602.3210) -- (243.8210,602.3210) -- (243.8210,587.3940) --
cycle(239.0310,602.3210) -- (243.8210,587.3940)(239.1420,587.3940) --
(243.8210,602.3210)(217.5820,546.8440) -- (212.7910,546.8440) --
(212.7910,555.5315) -- (217.5820,555.5315) -- (217.5820,546.8440) --
cycle(212.7910,555.5310) -- (217.5820,546.8440)(212.9020,546.8440) --
(217.5820,555.5310)(246.3240,546.8440) -- (241.5340,546.8440) --
(241.5340,555.5315) -- (246.3240,555.5315) -- (246.3240,546.8440) --
cycle(241.5340,555.5310) -- (246.3240,546.8440)(241.6450,546.8440) --
(246.3240,555.5310)(217.5820,488.0800) -- (212.7910,488.0800) --
(212.7910,496.7670) -- (217.5820,496.7670) -- (217.5820,488.0800) --
cycle(212.7910,496.7670) -- (217.5820,488.0800)(212.9020,488.0800) --
(217.5820,496.7670)(246.3240,488.0800) -- (241.5340,488.0800) --
(241.5340,496.7670) -- (246.3240,496.7670) -- (246.3240,488.0800) --
cycle(241.5340,496.7670) -- (246.3240,488.0800)(241.6450,488.0800) --
(246.3240,496.7670)(217.5820,461.2320) -- (212.7910,461.2320) --
(212.7910,469.9190) -- (217.5820,469.9190) -- (217.5820,461.2320) --
cycle(212.7910,469.9190) -- (217.5820,461.2320)(212.9020,461.2320) --
(217.5820,469.9190)(246.3240,461.2320) -- (241.5340,461.2320) --
(241.5340,469.9190) -- (246.3240,469.9190) -- (246.3240,461.2320) --
cycle(241.5340,469.9190) -- (246.3240,461.2320)(241.6450,461.2320) --
(246.3240,469.9190)(217.5820,435.0540) -- (212.7910,435.0540) --
(212.7910,443.7420) -- (217.5820,443.7420) -- (217.5820,435.0540) --
cycle(212.7910,443.7420) -- (217.5820,435.0540)(212.9020,435.0540) --
(217.5820,443.7420)(246.3240,435.0540) -- (241.5340,435.0540) --
(241.5340,443.7420) -- (246.3240,443.7420) -- (246.3240,435.0540) --
cycle(241.5340,443.7420) -- (246.3240,435.0540)(241.6450,435.0540) --
(246.3240,443.7420)(217.5820,407.7510) -- (212.7910,407.7510) --
(212.7910,416.4390) -- (217.5820,416.4390) -- (217.5820,407.7510) --
cycle(212.7910,416.4390) -- (217.5820,407.7510)(212.9020,407.7510) --
(217.5820,416.4390)(246.3240,407.7510) -- (241.5340,407.7510) --
(241.5340,416.4390) -- (246.3240,416.4390) -- (246.3240,407.7510) --
cycle(241.5340,416.4390) -- (246.3240,407.7510)(241.6450,407.7510) --
(246.3240,416.4390)(217.5820,370.6620) -- (212.7910,370.6620) --
(212.7910,379.3490) -- (217.5820,379.3490) -- (217.5820,370.6620) --
cycle(212.7910,379.3490) -- (217.5820,370.6620)(212.9020,370.6620) --
(217.5820,379.3490)(246.3240,370.6620) -- (241.5340,370.6620) --
(241.5340,379.3490) -- (246.3240,379.3490) -- (246.3240,370.6620) --
cycle(241.5340,379.3490) -- (246.3240,370.6620)(241.6450,370.6620) --
(246.3240,379.3490)(217.5820,342.5840) -- (212.7910,342.5840) --
(212.7910,351.2720) -- (217.5820,351.2720) -- (217.5820,342.5840) --
cycle(212.7910,351.2720) -- (217.5820,342.5840)(212.9020,342.5840) --
(217.5820,351.2720)(246.3240,342.5840) -- (241.5340,342.5840) --
(241.5340,351.2720) -- (246.3240,351.2720) -- (246.3240,342.5840) --
cycle(241.5340,351.2720) -- (246.3240,342.5840)(241.6450,342.5840) --
(246.3240,351.2720)(229.4670,639.7080) -- (229.4670,306.5820);


\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,379.3490) {ISh};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,416.4390) {DPH2};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,443.7420) {DP22};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,469.9190) {DP21};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,496.7670) {DPH1};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,555.5310) {DP12};


\node[color=red!80!black, anchor=base west, yshift=0, xshift=-31.5] at (166.8500,626.0810) {OL};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,338.8890) {DStig};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,355.7310) {DSh};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,582.0560) {DP11};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,594.7750) {QPol};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,609.0010) {HPol};




\path[fill=c211e1f,nonzero rule] (229.4670,303.5640) .. controls
(228.9400,304.9840) and (228.0410,306.7460) .. (227.0900,307.8370) --
(229.4670,306.9770) -- (231.8440,307.8370) .. controls (230.8930,306.7460) and
(229.9930,304.9840) .. (229.4670,303.5640);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] 
(173.0060,322.0650)--(285.9290,322.0650)    %SAD Plane
(173.0060,626.0810) -- (285.9290,626.0810)  %Specimen Plane
(227.7460,632.2420) -- (231.4110,632.2420)
(227.7460,620.1720) -- (231.4110,620.1720)
%DSh and DStig
(165.9560,355.7310) -- (168.9040,355.7310) -- (168.9040,338.8890) -- (166.0970,338.8890)
(168.9040,347.1690) -- (171.9910,347.1690)
%HPol QPOL DP11
(165.9560,609.0010) -- (168.9040,609.0010) -- (168.9040,582.0560) -- (166.0970,582.0560)
(168.9040,594.7750) -- (171.9910,594.7750);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt,rounded corners=5pt, dashed, color=black]
(229.4670,626.0810) -- (275,620.0810) -- (275,585.9140) -- (202.8500,532.4150)--
(202.8500,472.0820) -- (256.1830,432.7480) -- (256.5170,391.9150) -- (229.4670,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt,rounded corners=5pt, dashed, color=red!80!black]
(229.4670,620.1720) -- (265,586.0810) -- (265,532.0820) -- (210.6840,471.9150) --
(210.6840,432.5820) -- (249.1840,391.5820) -- (270.8500,322.0650);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=black,rounded corners=5pt]
(250,626.0810) -- (250,585.9140) -- (219,532.4150)--
(180,472.0820) -- (260,432.7480) -- (275,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=red!80!black,rounded corners=5pt]
(229.4670,626.0810)-- (275,586.0810) -- (265,532.0820) --  (245,471.9150) -- 
(180,432.5820) -- (229.4670,322.0650);

%\path[cm={{1.0,0.0,0.0,-1.0,(147.9459,631.6819)}},fill=c211e1f,nonzero rule]
%(0.0000,0.0000) node[above right] (text6164) {OL pre ffp
%specimen plane bfp HPol QPol DP11 DP12
%TL11 TL12 HP1 TL21 TL22 HP2
%ADL SAD plane DPH1 DPH2 lSh DSh
%DStig DP21 DP22 OL post};




\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,632.2420) {ffp};
\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,620.1720) {bfp};


\end{scope}
\end{tikzpicture}


==> for arxiv 2/figures/cetcor/cetcor_old.tex <==
\definecolor{cb4b6b9}{RGB}{180,182,185}
\definecolor{c211e1f}{RGB}{33,30,31}
\definecolor{c77797b}{RGB}{119,121,123}
\def\y1{0.5}
\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-\y1, xscale=1.000000, inner sep=0pt, outer sep=0pt]
	\begin{scope}[cm={{2.062,0.0,0.0,-2.062,(-129.99548,1482.0161)}}]
	
%ol
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (280.9290,626.1980) .. controls					
	(280.9290,618.7370) and (252.3650,612.6880) .. (229.4670,612.6880) .. controls
	(206.5680,612.6880) and (178.0060,618.7370) .. (178.0060,626.1980) .. controls
	(178.0060,633.6590) and (206.5680,639.7080) .. (229.4670,639.7080) .. controls
	(252.3650,639.7080) and (280.9290,633.6590) .. (280.9290,626.1980);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line width=0.400pt] 
(280.9290,626.1980) .. controls (280.9290,618.7370) and
(252.3650,612.6880) .. (229.4670,612.6880) .. controls (206.5680,612.6880) and
(178.0060,618.7370) .. (178.0060,626.1980) .. controls (178.0060,633.6590) and
(206.5680,639.7080) .. (229.4670,639.7080) .. controls (252.3650,639.7080) and
(280.9290,633.6590) .. (280.9290,626.1980) -- cycle;


\path[fill=cb4b6b9,nonzero rule] (283.7750,586.0280) .. controls
(283.7750,582.2590) and (248.4730,579.2040) .. (229.5980,579.2040) .. controls
(210.7230,579.2040) and (175.4200,582.2590) .. (175.4200,586.0280) .. controls
(175.4200,589.7960) and (210.7230,592.8500) .. (229.5980,592.8500) .. controls
(248.4730,592.8500) and (283.7750,589.7960) .. (283.7750,586.0280);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.7750,586.0280) .. controls (283.7750,582.2590) and
(248.4730,579.2040) .. (229.5980,579.2040) .. controls (210.7230,579.2040) and
(175.4200,582.2590) .. (175.4200,586.0280) .. controls (175.4200,589.7960) and
(210.7230,592.8500) .. (229.5980,592.8500) .. controls (248.4730,592.8500) and
(283.7750,589.7960) .. (283.7750,586.0280) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.0290,532.5260) .. controls
(283.0290,528.8980) and (248.7270,525.9580) .. (229.8510,525.9580) .. controls
(210.9750,525.9580) and (175.6740,528.8980) .. (175.6740,532.5260) .. controls
(175.6740,536.1530) and (210.9750,539.0930) .. (229.8510,539.0930) .. controls
(248.7270,539.0930) and (283.0290,536.1530) .. (283.0290,532.5260);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.0290,532.5260) .. controls (283.0290,528.8980) and
(248.7270,525.9580) .. (229.8510,525.9580) .. controls (210.9750,525.9580) and
(175.6740,528.8980) .. (175.6740,532.5260) .. controls (175.6740,536.1530) and
(210.9750,539.0930) .. (229.8510,539.0930) .. controls (248.7270,539.0930) and
(283.0290,536.1530) .. (283.0290,532.5260) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.9060,472.3160) .. controls
(283.9060,468.6220) and (248.6320,465.6260) .. (229.7890,465.6260) .. controls
(210.9470,465.6260) and (175.6720,468.6220) .. (175.6720,472.3160) .. controls
(175.6720,476.0110) and (210.9470,479.0060) .. (229.7890,479.0060) .. controls
(248.6320,479.0060) and (283.9060,476.0110) .. (283.9060,472.3160);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,472.3160) .. controls (283.9060,468.6220) and
(248.6320,465.6260) .. (229.7890,465.6260) .. controls (210.9470,465.6260) and
(175.6720,468.6220) .. (175.6720,472.3160) .. controls (175.6720,476.0110) and
(210.9470,479.0060) .. (229.7890,479.0060) .. controls (248.6320,479.0060) and
(283.9060,476.0110) .. (283.9060,472.3160) -- cycle;
\path[fill=cb4b6b9,nonzero rule] (283.9060,432.8440) .. controls
(283.9060,429.1500) and (248.6320,426.1550) .. (229.7890,426.1550) .. controls
(210.9470,426.1550) and (175.6720,429.1500) .. (175.6720,432.8440) .. controls
(175.6720,436.5390) and (210.9470,439.5350) .. (229.7890,439.5350) .. controls
(248.6320,439.5350) and (283.9060,436.5390) .. (283.9060,432.8440);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,432.8440) .. controls (283.9060,429.1500) and
(248.6320,426.1550) .. (229.7890,426.1550) .. controls (210.9470,426.1550) and
(175.6720,429.1500) .. (175.6720,432.8440) .. controls (175.6720,436.5390) and
(210.9470,439.5350) .. (229.7890,439.5350) .. controls (248.6320,439.5350) and
(283.9060,436.5390) .. (283.9060,432.8440) -- cycle;
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,391.8650) .. controls
(283.9060,388.1700) and (248.6320,385.1750) .. (229.7890,385.1750) .. controls
(210.9470,385.1750) and (175.6720,388.1700) .. (175.6720,391.8650) .. controls
(175.6720,395.5590) and (210.9470,398.5550) .. (229.7890,398.5550) .. controls
(248.6320,398.5550) and (283.9060,395.5590) .. (283.9060,391.8650);


\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,391.8650) {ADL};
\node[color=red!80!black, anchor=base west, yshift=6*\y1, xshift=5] at (286.9230,406.0820) {HP2};
\node[color=red!80!black, anchor=base west, yshift=8*\y1, xshift=5] at (286.9230,486.2910) {HP1};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,432.8440) {TL22};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,472.3160) {Tl21};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,532.5260) {TL12};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,586.0280) {TL11};

\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,322.0650) {SAD plane};
\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,626.0810) {specimen plane};


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,391.8650) .. controls (283.9060,388.1700) and
(248.6320,385.1750) .. (229.7890,385.1750) .. controls (210.9470,385.1750) and
(175.6720,388.1700) .. (175.6720,391.8650) .. controls (175.6720,395.5590) and
(210.9470,398.5550) .. (229.7890,398.5550) .. controls (248.6320,398.5550) and
(283.9060,395.5590) .. (283.9060,391.8650) -- cycle;
\path[fill=c77797b,nonzero rule] (175.7070,486.2910) -- (283.8730,486.2910) --
(283.8730,498.3750) -- (175.7070,498.3750) -- (175.7070,486.2910) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,486.2910) -- (175.7070,486.2910) --
(175.7070,498.3750) -- (283.8730,498.3750) -- (283.8730,486.2910) -- cycle;
\path[fill=c77797b,nonzero rule] (175.7070,406.0820) -- (283.8730,406.0820) --
(283.8730,418.1660) -- (175.7070,418.1660) -- (175.7070,406.0820) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,406.0820) -- (175.7070,406.0820) --
(175.7070,418.1660) -- (283.8730,418.1660) -- (283.8730,406.0820) --
cycle(220.2560,587.3940) -- (215.4649,587.3940) -- (215.4649,602.3210) --
(220.2560,602.3210) -- (220.2560,587.3940) -- cycle(215.4650,602.3210) --
(220.2560,587.3940)(215.5760,587.3940) --
(220.2560,602.3210)(243.8210,587.3940) -- (239.0309,587.3940) --
(239.0309,602.3210) -- (243.8210,602.3210) -- (243.8210,587.3940) --
cycle(239.0310,602.3210) -- (243.8210,587.3940)(239.1420,587.3940) --
(243.8210,602.3210)(217.5820,546.8440) -- (212.7910,546.8440) --
(212.7910,555.5315) -- (217.5820,555.5315) -- (217.5820,546.8440) --
cycle(212.7910,555.5310) -- (217.5820,546.8440)(212.9020,546.8440) --
(217.5820,555.5310)(246.3240,546.8440) -- (241.5340,546.8440) --
(241.5340,555.5315) -- (246.3240,555.5315) -- (246.3240,546.8440) --
cycle(241.5340,555.5310) -- (246.3240,546.8440)(241.6450,546.8440) --
(246.3240,555.5310)(217.5820,488.0800) -- (212.7910,488.0800) --
(212.7910,496.7670) -- (217.5820,496.7670) -- (217.5820,488.0800) --
cycle(212.7910,496.7670) -- (217.5820,488.0800)(212.9020,488.0800) --
(217.5820,496.7670)(246.3240,488.0800) -- (241.5340,488.0800) --
(241.5340,496.7670) -- (246.3240,496.7670) -- (246.3240,488.0800) --
cycle(241.5340,496.7670) -- (246.3240,488.0800)(241.6450,488.0800) --
(246.3240,496.7670)(217.5820,461.2320) -- (212.7910,461.2320) --
(212.7910,469.9190) -- (217.5820,469.9190) -- (217.5820,461.2320) --
cycle(212.7910,469.9190) -- (217.5820,461.2320)(212.9020,461.2320) --
(217.5820,469.9190)(246.3240,461.2320) -- (241.5340,461.2320) --
(241.5340,469.9190) -- (246.3240,469.9190) -- (246.3240,461.2320) --
cycle(241.5340,469.9190) -- (246.3240,461.2320)(241.6450,461.2320) --
(246.3240,469.9190)(217.5820,435.0540) -- (212.7910,435.0540) --
(212.7910,443.7420) -- (217.5820,443.7420) -- (217.5820,435.0540) --
cycle(212.7910,443.7420) -- (217.5820,435.0540)(212.9020,435.0540) --
(217.5820,443.7420)(246.3240,435.0540) -- (241.5340,435.0540) --
(241.5340,443.7420) -- (246.3240,443.7420) -- (246.3240,435.0540) --
cycle(241.5340,443.7420) -- (246.3240,435.0540)(241.6450,435.0540) --
(246.3240,443.7420)(217.5820,407.7510) -- (212.7910,407.7510) --
(212.7910,416.4390) -- (217.5820,416.4390) -- (217.5820,407.7510) --
cycle(212.7910,416.4390) -- (217.5820,407.7510)(212.9020,407.7510) --
(217.5820,416.4390)(246.3240,407.7510) -- (241.5340,407.7510) --
(241.5340,416.4390) -- (246.3240,416.4390) -- (246.3240,407.7510) --
cycle(241.5340,416.4390) -- (246.3240,407.7510)(241.6450,407.7510) --
(246.3240,416.4390)(217.5820,370.6620) -- (212.7910,370.6620) --
(212.7910,379.3490) -- (217.5820,379.3490) -- (217.5820,370.6620) --
cycle(212.7910,379.3490) -- (217.5820,370.6620)(212.9020,370.6620) --
(217.5820,379.3490)(246.3240,370.6620) -- (241.5340,370.6620) --
(241.5340,379.3490) -- (246.3240,379.3490) -- (246.3240,370.6620) --
cycle(241.5340,379.3490) -- (246.3240,370.6620)(241.6450,370.6620) --
(246.3240,379.3490)(217.5820,342.5840) -- (212.7910,342.5840) --
(212.7910,351.2720) -- (217.5820,351.2720) -- (217.5820,342.5840) --
cycle(212.7910,351.2720) -- (217.5820,342.5840)(212.9020,342.5840) --
(217.5820,351.2720)(246.3240,342.5840) -- (241.5340,342.5840) --
(241.5340,351.2720) -- (246.3240,351.2720) -- (246.3240,342.5840) --
cycle(241.5340,351.2720) -- (246.3240,342.5840)(241.6450,342.5840) --
(246.3240,351.2720)(229.4670,639.7080) -- (229.4670,306.5820);


\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,379.3490) {ISh};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,416.4390) {DPH2};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,443.7420) {DP22};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,469.9190) {DP21};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,496.7670) {DPH1};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,555.5310) {DP12};


\node[color=red!80!black, anchor=base west, yshift=0, xshift=-31.5] at (166.8500,626.0810) {OL};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,338.8890) {DStig};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,355.7310) {DSh};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,582.0560) {DP11};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,594.7750) {QPol};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,609.0010) {HPol};




\path[fill=c211e1f,nonzero rule] (229.4670,303.5640) .. controls
(228.9400,304.9840) and (228.0410,306.7460) .. (227.0900,307.8370) --
(229.4670,306.9770) -- (231.8440,307.8370) .. controls (230.8930,306.7460) and
(229.9930,304.9840) .. (229.4670,303.5640);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] 
(173.0060,322.0650)--(285.9290,322.0650)    %SAD Plane
(173.0060,626.0810) -- (285.9290,626.0810)  %Specimen Plane
(227.7460,632.2420) -- (231.4110,632.2420)
(227.7460,620.1720) -- (231.4110,620.1720)
%DSh and DStig
(165.9560,355.7310) -- (168.9040,355.7310) -- (168.9040,338.8890) -- (166.0970,338.8890)
(168.9040,347.1690) -- (171.9910,347.1690)
%HPol QPOL DP11
(165.9560,609.0010) -- (168.9040,609.0010) -- (168.9040,582.0560) -- (166.0970,582.0560)
(168.9040,594.7750) -- (171.9910,594.7750);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt,rounded corners=5pt, dashed, color=black]
(229.4670,626.0810) -- (275,620.0810) -- (275,585.9140) -- (202.8500,532.4150)--
(202.8500,472.0820) -- (256.1830,432.7480) -- (256.5170,391.9150) -- (229.4670,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt,rounded corners=5pt, dashed, color=red!80!black]
(229.4670,620.1720) -- (265,586.0810) -- (265,532.0820) -- (210.6840,471.9150) --
(210.6840,432.5820) -- (249.1840,391.5820) -- (270.8500,322.0650);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=black,rounded corners=5pt]
(250,626.0810) -- (250,585.9140) -- (219,532.4150)--
(180,472.0820) -- (260,432.7480) -- (275,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=red!80!black,rounded corners=5pt]
(229.4670,626.0810)-- (275,586.0810) -- (265,532.0820) --  (245,471.9150) -- 
(180,432.5820) -- (229.4670,322.0650);

%\path[cm={{1.0,0.0,0.0,-1.0,(147.9459,631.6819)}},fill=c211e1f,nonzero rule]
%(0.0000,0.0000) node[above right] (text6164) {OL pre ffp
%specimen plane bfp HPol QPol DP11 DP12
%TL11 TL12 HP1 TL21 TL22 HP2
%ADL SAD plane DPH1 DPH2 lSh DSh
%DStig DP21 DP22 OL post};




\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,632.2420) {ffp};
\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,620.1720) {bfp};


\end{scope}
\end{tikzpicture}


==> for arxiv 2/figures/chamber/chamber.tex <==
\pgfmathsetlength{\imagewidth}{\columnwidth}
\pgfmathsetlength{\imagescale}{\imagewidth/1024}

\begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
  \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0) {\includegraphics[width=\imagewidth]{figures/chamber/specimen_chamber.jpg}};
  \draw[ultra thick,white] (772,800) node [anchor=south west] {100\:mm} -- (1000,800);
  \draw[thick,color=orange] (505,380) circle (2.49cm); 
  \node[orange] at (30,370) [anchor=west] {permalloy} ;
  \node[orange] at (30,410) [anchor=west] {shielding} ;
  \node[yellow] at (850,100) [anchor=north] {ISO-K\:63 ports} ;
    \node[yellow] at (512,790) [anchor=north] {IGP port} ;
\end{tikzpicture}%


==> for arxiv 2/figures/chamber/chamber_old.tex <==
\pgfmathsetlength{\imagewidth}{\columnwidth}
\pgfmathsetlength{\imagescale}{\imagewidth/1024}

\begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
  \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0) {\includegraphics[width=\imagewidth]{figures/chamber/specimen_chamber.jpg}};
  \draw[ultra thick,white] (772,800) node [anchor=south west] {100\:mm} -- (1000,800);
  \node[yellow] at (850,100) [anchor=north] {ISO-K\:63 ports} ;
    \node[yellow] at (512,790) [anchor=north] {IGP port} ;
\end{tikzpicture}%


==> for arxiv 2/figures/cryo_layout/cryo_layout.tex <==

    \pgfmathsetlength{\imagewidth}{\columnwidth}
    \pgfmathsetlength{\imagescale}{\imagewidth/1024}

    \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\columnwidth]{figures/cryo_as_delivered}};
        \node[anchor=north west] at (0,0) {(a)};
        \draw [->, thick,red] (200,100) node[anchor=south]{electron beam hole} -- (240,280) ;
        \draw [->, thick] (450,150) node[anchor=south]{cooled radiation shield} -- (350,300) ;
        \draw [->, thick] (700,50) node[anchor=east]{liquid helium} -- (780,40) ;
        \draw [->, thick,yellow] (880,450) node[anchor=north]{helium exhaust} -- (880,380) ;
        \draw [->, thick,yellow] (450,450) node[anchor=north east]{auxiliary feedthrough ports} -- (660,240) ;
        \draw [->, thick,yellow] (460,460) -- (600,390) ;
      \end{tikzpicture}%
\vskip1ex
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\columnwidth]{figures/cryo_inner}};
        \node[anchor=north west] at (0,-200) {(b)};
        \draw [->, thick] (350,-100) node[anchor=south]{ring-shaped sample mount on stage} -- (500,110) ;
        \draw [->, thick] (650,-50) node[anchor=south]{4 cooled electrical terminals} -- (630,110) ;
        \draw [->, thick] (900,-100) node[anchor=south]{cold finger} -- (970,110) ;
        \draw [->, thick] (500,350) node[anchor=north]{space for additions} -- (200,200) ;
        \draw [->, thick] (524,350)  -- (800,200) ;
        \draw [ultra thick] (750,350) node[anchor=south west]{50 mm} -- (1000,350) ;
      \end{tikzpicture}%


==> for arxiv 2/figures/cryo_resolution/cryo_resolution.tex <==
\pgfmathsetlength{\imagewidth}{.49\columnwidth}
\pgfmathsetlength{\imagescale}{\imagewidth/1024}
%\centering
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{figures/cryo_resolution/160511_catalase_cold_0038}};
        \draw[ultra thick,white] (24,1000) node [anchor=south west] {100\:nm} -- (320,1000);
        \node at (0,0) [anchor=north west,white] {(a)} ;
%%         \draw[thick] (371,263) rectangle (474,366);
%%         \draw[] (371,263) -- (512,0);
%%         \draw[] (371,366) -- (512,512);
%%         \draw[] (474,263) -- (1024,0);
%%         \draw[] (474,366) -- (1024,512);
%%         \draw[thick] (371,263) rectangle (474,366);

%%         \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (512,0)
%%         {\includegraphics[width=.5\imagewidth]{../figures/tembench/140305_0024_calibrated_cut}};
%%         \draw[ultra thick] (536,488) node [anchor=south west] {10\:nm} -- (792,488);
%%         \draw[thick] (512,2) rectangle (1022,512);
      \end{tikzpicture}%
      \hfill
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{figures/cryo_resolution/160511_catalase_cold_0038F_contrast}};
        \draw[thick,dashed] (512,512) circle (275);
        \node at (512,237) [anchor=south west] {5\:nm} ;
        \draw[ultra thick] (24,1000) node [anchor=south west] {0.2\:nm$^{\text{--1}}$} -- (300,1000);
        \node at (0,0) [anchor=north west] {(b)} ;
      \end{tikzpicture}%


==> for arxiv 2/figures/cryo_resolution/tembench.tex <==
\pgfmathsetlength{\imagewidth}{.49\columnwidth}
\pgfmathsetlength{\imagescale}{\imagewidth/1024}
%\centering
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
      \tiny
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{../figures/tembench/140305_0024_calibrated_scaled}};
        \draw[ultra thick] (24,1000) node [anchor=south west] {50\:nm} -- (280,1000);
%        \node at (0,0) [anchor=north west] {(a)} ;
        \draw[thick] (371,263) rectangle (474,366);
        \draw[] (371,263) -- (512,0);
        \draw[] (371,366) -- (512,512);
        \draw[] (474,263) -- (1024,0);
        \draw[] (474,366) -- (1024,512);
        \draw[thick] (371,263) rectangle (474,366);

        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (512,0)
        {\includegraphics[width=.5\imagewidth]{../figures/tembench/140305_0024_calibrated_cut}};
        \draw[ultra thick] (536,488) node [anchor=south west] {10\:nm} -- (792,488);
        \draw[thick] (512,2) rectangle (1022,512);
      \end{tikzpicture}%
      \hfill
      \begin{tikzpicture}[x=\imagescale,y=-\imagescale]
      \sffamily
      \tiny
        \node[anchor=north west,inner sep=0pt,outer sep=0pt] at (0,0)
        {\includegraphics[width=\imagewidth]{../figures/tembench/young_lorentz_plain}};
        \draw[thick,dashed,white] (512,512) circle (360);
        \node at (512,152) [anchor=south west, white] {1.1\:nm} ;
        \draw[ultra thick,white] (24,1000) node [anchor=south west, white] {1\:nm$^{\text{--1}}$} -- (424,1000);
 %       \node at (0,0) [anchor=north west, white] {(b)} ;
      \end{tikzpicture}%


==> for arxiv 2/figures/darkfield/darkfield.tex <==
%\subfloat[Alternative darkfield imaging mode \label{fig:darkfield}]{
%Matrix Optics darkfield paper.py


\definecolor{dGray}{gray}{0.7}
\definecolor{lGray}{gray}{0.9}
\definecolor{cb4b6b9}{RGB}{180,182,185}
\definecolor{c211e1f}{RGB}{33,30,31}
\definecolor{c77797b}{RGB}{119,121,123}
\def\y1{0.5}


\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-\y1, xscale=0.8, inner sep=0pt, outer sep=0pt]
	\begin{scope}[cm={{2.062,0.0,0.0,-2.062,(-129.99548,1482.0161)}}]
	


%tl11
\path[fill=cb4b6b9,nonzero rule,color=lightgray] (283.7750,586.0280) .. controls
(283.7750,582.2590) and (248.4730,579.2040) .. (229.5980,579.2040) .. controls
(210.7230,579.2040) and (175.4200,582.2590) .. (175.4200,586.0280) .. controls
(175.4200,589.7960) and (210.7230,592.8500) .. (229.5980,592.8500) .. controls
(248.4730,592.8500) and (283.7750,589.7960) .. (283.7750,586.0280);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.7750,586.0280) .. controls (283.7750,582.2590) and
(248.4730,579.2040) .. (229.5980,579.2040) .. controls (210.7230,579.2040) and
(175.4200,582.2590) .. (175.4200,586.0280) .. controls (175.4200,589.7960) and
(210.7230,592.8500) .. (229.5980,592.8500) .. controls (248.4730,592.8500) and
(283.7750,589.7960) .. (283.7750,586.0280) -- cycle;

%tl12
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.0290,532.5260) .. controls
(283.0290,528.8980) and (248.7270,525.9580) .. (229.8510,525.9580) .. controls
(210.9750,525.9580) and (175.6740,528.8980) .. (175.6740,532.5260) .. controls
(175.6740,536.1530) and (210.9750,539.0930) .. (229.8510,539.0930) .. controls
(248.7270,539.0930) and (283.0290,536.1530) .. (283.0290,532.5260);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.0290,532.5260) .. controls (283.0290,528.8980) and
(248.7270,525.9580) .. (229.8510,525.9580) .. controls (210.9750,525.9580) and
(175.6740,528.8980) .. (175.6740,532.5260) .. controls (175.6740,536.1530) and
(210.9750,539.0930) .. (229.8510,539.0930) .. controls (248.7270,539.0930) and
(283.0290,536.1530) .. (283.0290,532.5260) -- cycle;

%Tl21
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,472.3160) .. controls
(283.9060,468.6220) and (248.6320,465.6260) .. (229.7890,465.6260) .. controls
(210.9470,465.6260) and (175.6720,468.6220) .. (175.6720,472.3160) .. controls
(175.6720,476.0110) and (210.9470,479.0060) .. (229.7890,479.0060) .. controls
(248.6320,479.0060) and (283.9060,476.0110) .. (283.9060,472.3160);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,472.3160) .. controls (283.9060,468.6220) and
(248.6320,465.6260) .. (229.7890,465.6260) .. controls (210.9470,465.6260) and
(175.6720,468.6220) .. (175.6720,472.3160) .. controls (175.6720,476.0110) and
(210.9470,479.0060) .. (229.7890,479.0060) .. controls (248.6320,479.0060) and
(283.9060,476.0110) .. (283.9060,472.3160) -- cycle;

%Tl22
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,432.8440) .. controls
(283.9060,429.1500) and (248.6320,426.1550) .. (229.7890,426.1550) .. controls
(210.9470,426.1550) and (175.6720,429.1500) .. (175.6720,432.8440) .. controls
(175.6720,436.5390) and (210.9470,439.5350) .. (229.7890,439.5350) .. controls
(248.6320,439.5350) and (283.9060,436.5390) .. (283.9060,432.8440);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,432.8440) .. controls (283.9060,429.1500) and
(248.6320,426.1550) .. (229.7890,426.1550) .. controls (210.9470,426.1550) and
(175.6720,429.1500) .. (175.6720,432.8440) .. controls (175.6720,436.5390) and
(210.9470,439.5350) .. (229.7890,439.5350) .. controls (248.6320,439.5350) and
(283.9060,436.5390) .. (283.9060,432.8440) -- cycle;

%adl
\path[fill=cb4b6b9,nonzero rule,color=lightgray] (283.9060,391.8650) .. controls
(283.9060,388.1700) and (248.6320,385.1750) .. (229.7890,385.1750) .. controls
(210.9470,385.1750) and (175.6720,388.1700) .. (175.6720,391.8650) .. controls
(175.6720,395.5590) and (210.9470,398.5550) .. (229.7890,398.5550) .. controls
(248.6320,398.5550) and (283.9060,395.5590) .. (283.9060,391.8650);


\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,391.8650) {ADL};
\node[color=red!80!black, anchor=base west, yshift=6*\y1, xshift=5] at (286.9230,404.0820) {HP2};
\node[color=red!80!black, anchor=base west, yshift=8*\y1, xshift=5] at (286.9230,483.2910) {HP1};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,432.8440) {TL22};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,472.3160) {Tl21};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,532.5260) {TL12};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,586.0280) {TL11};

\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,322.0650) {SA plane};
\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,626.0810) {specimen};
%\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (260.9230,326) {SA plane};
%\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (260,630) {specimen plane};


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,391.8650) .. controls (283.9060,388.1700) and
(248.6320,385.1750) .. (229.7890,385.1750) .. controls (210.9470,385.1750) and
(175.6720,388.1700) .. (175.6720,391.8650) .. controls (175.6720,395.5590) and
(210.9470,398.5550) .. (229.7890,398.5550) .. controls (248.6320,398.5550) and
(283.9060,395.5590) .. (283.9060,391.8650) -- cycle;

%HP1
\path[fill=c77797b,nonzero rule,pattern=north west lines,pattern color=lightgray] (175.7070,486.2910) -- (283.8730,486.2910) --
(283.8730,498.3750) -- (175.7070,498.3750) -- (175.7070,486.2910) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,486.2910) -- (175.7070,486.2910) --
(175.7070,498.3750) -- (283.8730,498.3750) -- (283.8730,486.2910) -- cycle;
%HP2
\path[fill=c77797b,nonzero rule,pattern=north west lines,pattern color=lightgray] (175.7070,406.0820) -- (283.8730,406.0820) --
(283.8730,418.1660) -- (175.7070,418.1660) -- (175.7070,406.0820) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,406.0820) -- (175.7070,406.0820) --
(175.7070,418.1660) -- (283.8730,418.1660) -- (283.8730,406.0820) --
cycle(220.2560,587.3940) -- (215.4649,587.3940) -- (215.4649,602.3210) --
(220.2560,602.3210) -- (220.2560,587.3940) -- cycle(215.4650,602.3210) --
(220.2560,587.3940)
(215.5760,587.3940) --(220.2560,602.3210)
(243.8210,587.3940) -- (239.0309,587.3940) --
(239.0309,602.3210) -- (243.8210,602.3210) -- (243.8210,587.3940) --
cycle(239.0310,602.3210) -- (243.8210,587.3940)(239.1420,587.3940) --
(243.8210,602.3210)(217.5820,546.8440) -- (212.7910,546.8440) --
(212.7910,555.5315) -- (217.5820,555.5315) -- (217.5820,546.8440) --
cycle(212.7910,555.5310) -- (217.5820,546.8440)(212.9020,546.8440) --
(217.5820,555.5310)(246.3240,546.8440) -- (241.5340,546.8440) --
(241.5340,555.5315) -- (246.3240,555.5315) -- (246.3240,546.8440) --
cycle(241.5340,555.5310) -- (246.3240,546.8440)(241.6450,546.8440) --
(246.3240,555.5310)(217.5820,488.0800) -- (212.7910,488.0800) --
(212.7910,496.7670) -- (217.5820,496.7670) -- (217.5820,488.0800) --
cycle(212.7910,496.7670) -- (217.5820,488.0800)(212.9020,488.0800) --
(217.5820,496.7670)(246.3240,488.0800) -- (241.5340,488.0800) --
(241.5340,496.7670) -- (246.3240,496.7670) -- (246.3240,488.0800) --
cycle(241.5340,496.7670) -- (246.3240,488.0800)(241.6450,488.0800) --
(246.3240,496.7670)(217.5820,461.2320) -- (212.7910,461.2320) --
(212.7910,469.9190) -- (217.5820,469.9190) -- (217.5820,461.2320) --
cycle(212.7910,469.9190) -- (217.5820,461.2320)(212.9020,461.2320) --
(217.5820,469.9190)(246.3240,461.2320) -- (241.5340,461.2320) --
(241.5340,469.9190) -- (246.3240,469.9190) -- (246.3240,461.2320) --
cycle(241.5340,469.9190) -- (246.3240,461.2320)(241.6450,461.2320) --
(246.3240,469.9190)(217.5820,435.0540) -- (212.7910,435.0540) --
(212.7910,443.7420) -- (217.5820,443.7420) -- (217.5820,435.0540) --
cycle(212.7910,443.7420) -- (217.5820,435.0540)(212.9020,435.0540) --
(217.5820,443.7420)(246.3240,435.0540) -- (241.5340,435.0540) --
(241.5340,443.7420) -- (246.3240,443.7420) -- (246.3240,435.0540) --
cycle(241.5340,443.7420) -- (246.3240,435.0540)(241.6450,435.0540) --
(246.3240,443.7420)(217.5820,407.7510) -- (212.7910,407.7510) --
(212.7910,416.4390) -- (217.5820,416.4390) -- (217.5820,407.7510) --
cycle(212.7910,416.4390) -- (217.5820,407.7510)(212.9020,407.7510) --
(217.5820,416.4390)(246.3240,407.7510) -- (241.5340,407.7510) --
(241.5340,416.4390) -- (246.3240,416.4390) -- (246.3240,407.7510) --
cycle(241.5340,416.4390) -- (246.3240,407.7510)(241.6450,407.7510) --
(246.3240,416.4390)(217.5820,370.6620) -- (212.7910,370.6620) --
(212.7910,379.3490) -- (217.5820,379.3490) -- (217.5820,370.6620) --
cycle(212.7910,379.3490) -- (217.5820,370.6620)(212.9020,370.6620) --
(217.5820,379.3490)(246.3240,370.6620) -- (241.5340,370.6620) --
(241.5340,379.3490) -- (246.3240,379.3490) -- (246.3240,370.6620) --
cycle(241.5340,379.3490) -- (246.3240,370.6620)(241.6450,370.6620) --
(246.3240,379.3490)(217.5820,342.5840) -- (212.7910,342.5840) --
(212.7910,351.2720) -- (217.5820,351.2720) -- (217.5820,342.5840) --
cycle(212.7910,351.2720) -- (217.5820,342.5840)(212.9020,342.5840) --
(217.5820,351.2720)(246.3240,342.5840) -- (241.5340,342.5840) --
(241.5340,351.2720) -- (246.3240,351.2720) -- (246.3240,342.5840) --
cycle(241.5340,351.2720) -- (246.3240,342.5840)(241.6450,342.5840) --
(246.3240,351.2720)
(229.4670,626.0810) -- (229.4670,306.5820);


\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,379.3490) {ISh};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,416.4390) {DPH2};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,443.7420) {DP22};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,469.9190) {DP21};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,496.7670) {DPH1};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,555.5310) {DP12};


\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,338.8890) {DStig};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,355.7310) {DSh};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,582.0560) {DP11};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,594.7750) {QPol};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,609.0010) {HPol};




\path[fill=c211e1f,nonzero rule] (229.4670,303.5640) .. controls
(228.9400,304.9840) and (228.0410,306.7460) .. (227.0900,307.8370) --
(229.4670,306.9770) -- (231.8440,307.8370) .. controls (230.8930,306.7460) and
(229.9930,304.9840) .. (229.4670,303.5640);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] 
(173.0060,322.0650)--(285.9290,322.0650)    %SAD Plane
(173.0060,626.0810) -- (285.9290,626.0810)  %Specimen Plane

%bfp ffp
%(227.7460,632.2420) -- (231.4110,632.2420)
%(227.7460,620.1720) -- (231.4110,620.1720)
%DSh and DStig
(165.9560,355.7310) -- (168.9040,355.7310) -- (168.9040,338.8890) -- (166.0970,338.8890)
(168.9040,347.1690) -- (171.9910,347.1690)
%HPol QPOL DP11
(165.9560,609.0010) -- (168.9040,609.0010) -- (168.9040,582.0560) -- (166.0970,582.0560)
(168.9040,594.7750) -- (171.9910,594.7750);


%\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
%width=0.400pt,rounded corners=5pt, dashed, color=black]
%(229.4670,626.0810) -- (275,620.0810) -- (275,585.9140) -- (202.8500,532.4150)--
%(202.8500,472.0820) -- (256.1830,432.7480) -- (256.5170,391.9150) -- (229.4670,322.0650);

%\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
%width=0.400pt,rounded corners=5pt, dashed, color=red!80!black]
%(229.4670,620.1720) -- (265,586.0810) -- (265,532.0820) -- (210.6840,471.9150) --
%(210.6840,432.5820) -- (249.1840,391.5820) -- (270.8500,322.0650);


%beam
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=black,rounded corners=5pt]
(249.4670,626.0810) -- (249.4670,585.9140) -- (180,390) -- (229.4670,322.0650);

%beam
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=red!80!black,rounded corners=5pt]
(229.4670,626.0810)-- (255,586.0810) -- (235,390) -- (215,322.0650)
(249.4670,626.0810)-- (275,586.0810) -- (182,390) -- (215,322.0650);


%\path[cm={{1.0,0.0,0.0,-1.0,(147.9459,631.6819)}},fill=c211e1f,nonzero rule]
%(0.0000,0.0000) node[above right] (text6164) {OL pre ffp
%specimen plane bfp HPol QPol DP11 DP12
%TL11 TL12 HP1 TL21 TL22 HP2
%ADL SAD plane DPH1 DPH2 lSh DSh
%DStig DP21 DP22 OL post};




%\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,632.2420) {ffp};
%\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,620.1720) {bfp};


\end{scope}
\end{tikzpicture}



==> for arxiv 2/figures/darkfield/darkfield_old.tex <==
%\subfloat[Alternative darkfield imaging mode \label{fig:darkfield}]{
%Matrix Optics darkfield paper.py


\definecolor{dGray}{gray}{0.7}
\definecolor{lGray}{gray}{0.9}
\definecolor{cb4b6b9}{RGB}{180,182,185}
\definecolor{c211e1f}{RGB}{33,30,31}
\definecolor{c77797b}{RGB}{119,121,123}
\def\y1{0.5}


\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-\y1, xscale=1.000000, inner sep=0pt, outer sep=0pt]
	\begin{scope}[cm={{2.062,0.0,0.0,-2.062,(-129.99548,1482.0161)}}]
	
%ol
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (280.9290,626.1980) .. controls					
	(280.9290,618.7370) and (252.3650,612.6880) .. (229.4670,612.6880) .. controls
	(206.5680,612.6880) and (178.0060,618.7370) .. (178.0060,626.1980) .. controls
	(178.0060,633.6590) and (206.5680,639.7080) .. (229.4670,639.7080) .. controls
	(252.3650,639.7080) and (280.9290,633.6590) .. (280.9290,626.1980);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line width=0.400pt] 
(280.9290,626.1980) .. controls (280.9290,618.7370) and
(252.3650,612.6880) .. (229.4670,612.6880) .. controls (206.5680,612.6880) and
(178.0060,618.7370) .. (178.0060,626.1980) .. controls (178.0060,633.6590) and
(206.5680,639.7080) .. (229.4670,639.7080) .. controls (252.3650,639.7080) and
(280.9290,633.6590) .. (280.9290,626.1980) -- cycle;

%tl11
\path[fill=cb4b6b9,nonzero rule,color=lightgray] (283.7750,586.0280) .. controls
(283.7750,582.2590) and (248.4730,579.2040) .. (229.5980,579.2040) .. controls
(210.7230,579.2040) and (175.4200,582.2590) .. (175.4200,586.0280) .. controls
(175.4200,589.7960) and (210.7230,592.8500) .. (229.5980,592.8500) .. controls
(248.4730,592.8500) and (283.7750,589.7960) .. (283.7750,586.0280);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.7750,586.0280) .. controls (283.7750,582.2590) and
(248.4730,579.2040) .. (229.5980,579.2040) .. controls (210.7230,579.2040) and
(175.4200,582.2590) .. (175.4200,586.0280) .. controls (175.4200,589.7960) and
(210.7230,592.8500) .. (229.5980,592.8500) .. controls (248.4730,592.8500) and
(283.7750,589.7960) .. (283.7750,586.0280) -- cycle;

%tl12
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.0290,532.5260) .. controls
(283.0290,528.8980) and (248.7270,525.9580) .. (229.8510,525.9580) .. controls
(210.9750,525.9580) and (175.6740,528.8980) .. (175.6740,532.5260) .. controls
(175.6740,536.1530) and (210.9750,539.0930) .. (229.8510,539.0930) .. controls
(248.7270,539.0930) and (283.0290,536.1530) .. (283.0290,532.5260);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.0290,532.5260) .. controls (283.0290,528.8980) and
(248.7270,525.9580) .. (229.8510,525.9580) .. controls (210.9750,525.9580) and
(175.6740,528.8980) .. (175.6740,532.5260) .. controls (175.6740,536.1530) and
(210.9750,539.0930) .. (229.8510,539.0930) .. controls (248.7270,539.0930) and
(283.0290,536.1530) .. (283.0290,532.5260) -- cycle;

%Tl21
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,472.3160) .. controls
(283.9060,468.6220) and (248.6320,465.6260) .. (229.7890,465.6260) .. controls
(210.9470,465.6260) and (175.6720,468.6220) .. (175.6720,472.3160) .. controls
(175.6720,476.0110) and (210.9470,479.0060) .. (229.7890,479.0060) .. controls
(248.6320,479.0060) and (283.9060,476.0110) .. (283.9060,472.3160);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,472.3160) .. controls (283.9060,468.6220) and
(248.6320,465.6260) .. (229.7890,465.6260) .. controls (210.9470,465.6260) and
(175.6720,468.6220) .. (175.6720,472.3160) .. controls (175.6720,476.0110) and
(210.9470,479.0060) .. (229.7890,479.0060) .. controls (248.6320,479.0060) and
(283.9060,476.0110) .. (283.9060,472.3160) -- cycle;

%Tl22
\path[fill=cb4b6b9,nonzero rule,pattern=north west lines,pattern color=lightgray] (283.9060,432.8440) .. controls
(283.9060,429.1500) and (248.6320,426.1550) .. (229.7890,426.1550) .. controls
(210.9470,426.1550) and (175.6720,429.1500) .. (175.6720,432.8440) .. controls
(175.6720,436.5390) and (210.9470,439.5350) .. (229.7890,439.5350) .. controls
(248.6320,439.5350) and (283.9060,436.5390) .. (283.9060,432.8440);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,432.8440) .. controls (283.9060,429.1500) and
(248.6320,426.1550) .. (229.7890,426.1550) .. controls (210.9470,426.1550) and
(175.6720,429.1500) .. (175.6720,432.8440) .. controls (175.6720,436.5390) and
(210.9470,439.5350) .. (229.7890,439.5350) .. controls (248.6320,439.5350) and
(283.9060,436.5390) .. (283.9060,432.8440) -- cycle;

%adl
\path[fill=cb4b6b9,nonzero rule,color=lightgray] (283.9060,391.8650) .. controls
(283.9060,388.1700) and (248.6320,385.1750) .. (229.7890,385.1750) .. controls
(210.9470,385.1750) and (175.6720,388.1700) .. (175.6720,391.8650) .. controls
(175.6720,395.5590) and (210.9470,398.5550) .. (229.7890,398.5550) .. controls
(248.6320,398.5550) and (283.9060,395.5590) .. (283.9060,391.8650);


\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,391.8650) {ADL};
\node[color=red!80!black, anchor=base west, yshift=6*\y1, xshift=5] at (286.9230,404.0820) {HP2};
\node[color=red!80!black, anchor=base west, yshift=8*\y1, xshift=5] at (286.9230,483.2910) {HP1};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,432.8440) {TL22};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,472.3160) {Tl21};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,532.5260) {TL12};
\node[color=red!80!black, anchor=base west, yshift=-8*\y1, xshift=5] at (286.9230,586.0280) {TL11};

\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,322.0650) {SAD plane};
\node[color=red!80!black, anchor=base west, yshift=0, xshift=5] at (286.9230,626.0810) {specimen plane};


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.9060,391.8650) .. controls (283.9060,388.1700) and
(248.6320,385.1750) .. (229.7890,385.1750) .. controls (210.9470,385.1750) and
(175.6720,388.1700) .. (175.6720,391.8650) .. controls (175.6720,395.5590) and
(210.9470,398.5550) .. (229.7890,398.5550) .. controls (248.6320,398.5550) and
(283.9060,395.5590) .. (283.9060,391.8650) -- cycle;

%HP1
\path[fill=c77797b,nonzero rule,pattern=north west lines,pattern color=lightgray] (175.7070,486.2910) -- (283.8730,486.2910) --
(283.8730,498.3750) -- (175.7070,498.3750) -- (175.7070,486.2910) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,486.2910) -- (175.7070,486.2910) --
(175.7070,498.3750) -- (283.8730,498.3750) -- (283.8730,486.2910) -- cycle;
%HP2
\path[fill=c77797b,nonzero rule,pattern=north west lines,pattern color=lightgray] (175.7070,406.0820) -- (283.8730,406.0820) --
(283.8730,418.1660) -- (175.7070,418.1660) -- (175.7070,406.0820) -- cycle;
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] (283.8730,406.0820) -- (175.7070,406.0820) --
(175.7070,418.1660) -- (283.8730,418.1660) -- (283.8730,406.0820) --
cycle(220.2560,587.3940) -- (215.4649,587.3940) -- (215.4649,602.3210) --
(220.2560,602.3210) -- (220.2560,587.3940) -- cycle(215.4650,602.3210) --
(220.2560,587.3940)(215.5760,587.3940) --
(220.2560,602.3210)(243.8210,587.3940) -- (239.0309,587.3940) --
(239.0309,602.3210) -- (243.8210,602.3210) -- (243.8210,587.3940) --
cycle(239.0310,602.3210) -- (243.8210,587.3940)(239.1420,587.3940) --
(243.8210,602.3210)(217.5820,546.8440) -- (212.7910,546.8440) --
(212.7910,555.5315) -- (217.5820,555.5315) -- (217.5820,546.8440) --
cycle(212.7910,555.5310) -- (217.5820,546.8440)(212.9020,546.8440) --
(217.5820,555.5310)(246.3240,546.8440) -- (241.5340,546.8440) --
(241.5340,555.5315) -- (246.3240,555.5315) -- (246.3240,546.8440) --
cycle(241.5340,555.5310) -- (246.3240,546.8440)(241.6450,546.8440) --
(246.3240,555.5310)(217.5820,488.0800) -- (212.7910,488.0800) --
(212.7910,496.7670) -- (217.5820,496.7670) -- (217.5820,488.0800) --
cycle(212.7910,496.7670) -- (217.5820,488.0800)(212.9020,488.0800) --
(217.5820,496.7670)(246.3240,488.0800) -- (241.5340,488.0800) --
(241.5340,496.7670) -- (246.3240,496.7670) -- (246.3240,488.0800) --
cycle(241.5340,496.7670) -- (246.3240,488.0800)(241.6450,488.0800) --
(246.3240,496.7670)(217.5820,461.2320) -- (212.7910,461.2320) --
(212.7910,469.9190) -- (217.5820,469.9190) -- (217.5820,461.2320) --
cycle(212.7910,469.9190) -- (217.5820,461.2320)(212.9020,461.2320) --
(217.5820,469.9190)(246.3240,461.2320) -- (241.5340,461.2320) --
(241.5340,469.9190) -- (246.3240,469.9190) -- (246.3240,461.2320) --
cycle(241.5340,469.9190) -- (246.3240,461.2320)(241.6450,461.2320) --
(246.3240,469.9190)(217.5820,435.0540) -- (212.7910,435.0540) --
(212.7910,443.7420) -- (217.5820,443.7420) -- (217.5820,435.0540) --
cycle(212.7910,443.7420) -- (217.5820,435.0540)(212.9020,435.0540) --
(217.5820,443.7420)(246.3240,435.0540) -- (241.5340,435.0540) --
(241.5340,443.7420) -- (246.3240,443.7420) -- (246.3240,435.0540) --
cycle(241.5340,443.7420) -- (246.3240,435.0540)(241.6450,435.0540) --
(246.3240,443.7420)(217.5820,407.7510) -- (212.7910,407.7510) --
(212.7910,416.4390) -- (217.5820,416.4390) -- (217.5820,407.7510) --
cycle(212.7910,416.4390) -- (217.5820,407.7510)(212.9020,407.7510) --
(217.5820,416.4390)(246.3240,407.7510) -- (241.5340,407.7510) --
(241.5340,416.4390) -- (246.3240,416.4390) -- (246.3240,407.7510) --
cycle(241.5340,416.4390) -- (246.3240,407.7510)(241.6450,407.7510) --
(246.3240,416.4390)(217.5820,370.6620) -- (212.7910,370.6620) --
(212.7910,379.3490) -- (217.5820,379.3490) -- (217.5820,370.6620) --
cycle(212.7910,379.3490) -- (217.5820,370.6620)(212.9020,370.6620) --
(217.5820,379.3490)(246.3240,370.6620) -- (241.5340,370.6620) --
(241.5340,379.3490) -- (246.3240,379.3490) -- (246.3240,370.6620) --
cycle(241.5340,379.3490) -- (246.3240,370.6620)(241.6450,370.6620) --
(246.3240,379.3490)(217.5820,342.5840) -- (212.7910,342.5840) --
(212.7910,351.2720) -- (217.5820,351.2720) -- (217.5820,342.5840) --
cycle(212.7910,351.2720) -- (217.5820,342.5840)(212.9020,342.5840) --
(217.5820,351.2720)(246.3240,342.5840) -- (241.5340,342.5840) --
(241.5340,351.2720) -- (246.3240,351.2720) -- (246.3240,342.5840) --
cycle(241.5340,351.2720) -- (246.3240,342.5840)(241.6450,342.5840) --
(246.3240,351.2720)(229.4670,639.7080) -- (229.4670,306.5820);


\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,379.3490) {ISh};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,416.4390) {DPH2};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,443.7420) {DP22};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,469.9190) {DP21};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,496.7670) {DPH1};
\node[color=red!80!black, anchor=base west, yshift=-12*\y1, xshift=-30] at (166.0970,555.5310) {DP12};


\node[color=red!80!black, anchor=base west, yshift=0, xshift=-31.5] at (166.8500,626.0810) {OL};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,338.8890) {DStig};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,355.7310) {DSh};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,582.0560) {DP11};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,594.7750) {QPol};
\node[color=red!80!black, anchor=base west, yshift=-3, xshift=-30] at (166.0970,609.0010) {HPol};




\path[fill=c211e1f,nonzero rule] (229.4670,303.5640) .. controls
(228.9400,304.9840) and (228.0410,306.7460) .. (227.0900,307.8370) --
(229.4670,306.9770) -- (231.8440,307.8370) .. controls (230.8930,306.7460) and
(229.9930,304.9840) .. (229.4670,303.5640);
\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt] 
(173.0060,322.0650)--(285.9290,322.0650)    %SAD Plane
(173.0060,626.0810) -- (285.9290,626.0810)  %Specimen Plane

%bfp ffp
%(227.7460,632.2420) -- (231.4110,632.2420)
%(227.7460,620.1720) -- (231.4110,620.1720)
%DSh and DStig
(165.9560,355.7310) -- (168.9040,355.7310) -- (168.9040,338.8890) -- (166.0970,338.8890)
(168.9040,347.1690) -- (171.9910,347.1690)
%HPol QPOL DP11
(165.9560,609.0010) -- (168.9040,609.0010) -- (168.9040,582.0560) -- (166.0970,582.0560)
(168.9040,594.7750) -- (171.9910,594.7750);


%\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
%width=0.400pt,rounded corners=5pt, dashed, color=black]
%(229.4670,626.0810) -- (275,620.0810) -- (275,585.9140) -- (202.8500,532.4150)--
%(202.8500,472.0820) -- (256.1830,432.7480) -- (256.5170,391.9150) -- (229.4670,322.0650);

%\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
%width=0.400pt,rounded corners=5pt, dashed, color=red!80!black]
%(229.4670,620.1720) -- (265,586.0810) -- (265,532.0820) -- (210.6840,471.9150) --
%(210.6840,432.5820) -- (249.1840,391.5820) -- (270.8500,322.0650);


\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=black,rounded corners=5pt]
(249.4670,626.0810) -- (249.4670,585.9140) -- (180,390) -- (229.4670,322.0650);

\path[draw=c211e1f,line join=miter,line cap=butt,miter limit=4.00,line
width=0.400pt, color=red!80!black,rounded corners=5pt]
(229.4670,626.0810)-- (255,586.0810) -- (235,390) -- (215,322.0650)
(249.4670,626.0810)-- (275,586.0810) -- (182,390) -- (215,322.0650);


%\path[cm={{1.0,0.0,0.0,-1.0,(147.9459,631.6819)}},fill=c211e1f,nonzero rule]
%(0.0000,0.0000) node[above right] (text6164) {OL pre ffp
%specimen plane bfp HPol QPol DP11 DP12
%TL11 TL12 HP1 TL21 TL22 HP2
%ADL SAD plane DPH1 DPH2 lSh DSh
%DStig DP21 DP22 OL post};




%\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,632.2420) {ffp};
%\node[color=red!80!black, anchor=base west, yshift=-5*\y1, xshift=-23] at (231.4110,620.1720) {bfp};


\end{scope}
\end{tikzpicture}



==> for arxiv 2/figures/holo/holo.tex <==
\begin{tikzpicture}[xscale=0.7,yscale=0.5]
%\draw [help lines] (-5,-5) grid (5,5);




\def\t{0.5} 
\def\s{0.25}
\def\nub{5} % anz. der Strahlen


%undiffracted beam

\foreach \x in {1,3,5,...,\nub}    
	\draw [black, thick,rounded corners=8pt](0,6) -- (\x/2-1/2-\nub/4+1/4,3) -- (\x/2-1/2-\nub/4+1/4,0) -- (\x/2-1/2-\nub/4+1/4,-2) -- (-\x+1+\nub/2-1/2,-9) -- (-\x*1.25+\nub/2+1.25,-12);

%virtual beam 1

\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (1.35,-4.325) -- (0,0);
\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (-1.35,-4.325) -- (0,0);

\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (1.35,-4.325) -- (2.5,-12);
\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (1.35,-4.325) -- (-.5,-12);

\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (-1.35,-4.325) -- (-2.5,-12);
\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (-1.35,-4.325) -- (.5,-12);
\node[color=red!80!black] at (-1.65,-4.325+0.6) {$-\boldsymbol{\frac{q_c}{2}}$};
\node[color=red!80!black] at (1.6,-4.325+0.6) {$+\boldsymbol{\frac{q_c}{2}}$};
\filldraw[color=red!80!black] (-1.35-0.04,-4.325) arc (180:-180:0.0253/0.7 and 0.056); 
\filldraw[color=red!80!black] (1.35-0.04,-4.325) arc (180:-180:0.0253/0.7 and 0.056); 

%virtual beam 2
%\foreach \x in {1,5,...,\nub}    
%	\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (\x/1.5-1/2-\nub/4-1/4,-4.325) -- (\x-1-\nub/2+1/2,-9) -- (-2.5,-12);
%\foreach \x in {1,5,...,\nub}    
%	\draw [black,opacity=.7, thick,rounded corners=8pt,dotted] (\x/1.5-1/2-\nub/4-1/4,-4.325) -- (-\x/4+\nub/2-1.75,-12);


%diffracted beam  
\draw [red!80!black,opacity=.7, thick,rounded corners=8pt] (0.5,0)  -- (0.25,-2) -- (-1.1,-9) -- (-1,-12);
\draw [red!80!black,opacity=.7, thick,rounded corners=8pt] (0.5,0)  -- (0.75,-2) -- (-0.95,-9) -- (-1,-12);


%image and ref wave
%image
\fill [red!80!black,opacity=.3, thick,rounded corners=5pt] (0 ,0)  -- (0,-12.2) -- (-2.53,-12.2) -- (-2,-9) -- (1,-2) -- (1,0);
%ref
\fill [black,opacity=.3, thick,rounded corners=5pt] (0 ,0)  -- (0,-12.2) -- (2.53,-12.2) -- (2,-9) -- (-1,-2) -- (-1,0);


% annotation B
%\filldraw [fill=white ,draw=white] (3.3,{0.0+1}) circle (0.24) [path picture={ \node at (path picture bounding box.center) {$\color{red}\mathrm{\boldsymbol{B}}$};} ];
%\filldraw [fill=white ,draw=white] (3.3,{0.0-1}) circle (0.24) [path picture={ \node at (path picture bounding box.center) {$\color{red}\mathrm{\boldsymbol{B}}$};} ];


% biprism
\filldraw[draw=black, line width=0.25 ,fill=red!80!black] (-.18,-9)  arc (180:-180:0.125/0.7 and 0.25);
\filldraw[draw=black, line width=0.25 ,fill=red!80!black] (-3,-8.5) -- (-3,-9.5)--(-3.05,-9.5)--(-3.05,-8.5)--(-3,-8.5);
\filldraw[draw=black, line width=0.25 ,fill=red!80!black] (3,-8.5) -- (3,-9.5)--(3.05,-9.5)--(3.05,-8.5)--(3,-8.5);
\draw [black, line width=0.25] (3.05,-9.25)  -- (3.25,-9.25)-- (3.25,-9.75);
\draw [black, line width=0.25] (3.1,-9.75) -- (3.4,-9.75);
\draw [black, line width=0.25] (3.15,-9.85) -- (3.35,-9.85);
\draw [black, line width=0.25] (3.2,-9.95) -- (3.3,-9.95);

\draw [black, line width=0.25] (-3.05,-9.25)  -- (-3.25,-9.25)-- (-3.25,-9.75);
\draw [black, line width=0.25] (-3.1,-9.75) -- (-3.4,-9.75);
\draw [black, line width=0.25] (-3.15,-9.85) -- (-3.35,-9.85);
\draw [black, line width=0.25] (-3.2,-9.95) -- (-3.3,-9.95);


\draw [black, thick] (0.1,-9)  -- (-0.1,-9);
\draw [black, thick] (0,-9.14)  -- (0,-8.86);


%specimen, image and hologramm	

\filldraw[draw=black, line width=0.25 ,fill=red!80!black,rounded corners=0.3pt] (-0.025,0)--(2,0)--(2,0.2) --(-0.025,0.2)--(-0.025,0)--(2,0);
\filldraw[draw=black, line width=0.25 ,fill=red!80!black,rounded corners=0.3pt] (0.55,-12)--(-2.55,-12)--(-2.55,-12.2) --(0.55,-12.2)--(0.55,-12)--(-2.55,-12);
\def\anz{20}
\foreach \x in {0,1,2,...,\anz}    
	\draw [black,opacity=.7,rounded corners=8pt] (-0.5+\x/\anz,-12.2) -- (-0.5+\x/\anz,-12);



%lenses
%conderser
\fill[gray,opacity=.5] (-2,2.9)  arc (180:-180:2 and 0.2);
%main imaging lens
\fill[gray,opacity=.5] (-4,-1.9)  arc (180:-180:4 and 0.2);

%specimen plane

\draw [black,opacity=.7, thick,dashed] (-4,0) -- (4,0);
\node[color=red!80!black, anchor=base west] at (3,0.25) {specimen plane};

%backfocal plane

\draw [black,opacity=.7, thick,dashed] (-4,-4.325) -- (4,-4.325);
\node[color=red!80!black, anchor=base west] at (3,-4.325+0.25) {back focal plane};


%image plane

\draw [black,opacity=.7, thick,dashed] (-4,-12.2) -- (4,-12.2);
\node[color=red!80!black, anchor=base west] at (3,-12.2+0.25) {image plane};

%annotaions

\node[color=red!80!black, anchor=base west] at (-5.5,-9.125) {biprism};
\node[color=red!80!black, anchor=base west] at (-5.5,-2+0.5) {main imaging lens};
\node[color=red!80!black, anchor=base west] at (-5.5,3+0.1) {condenser system};
\node[color=red!80!black] at (0,-12-0.7) {hologramm};


\draw [<->] (1,-8.55) -- (3,-8.55) [-stealth, line width=0.25pt, black];
\draw [<->] (2,-8.55) -- (0,-8.55) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (1.1,-9.15) {$\mathrm{d_{bp}}$};


\draw [<->] (0.25,-11.8) -- (0.5,-11.8) [-stealth, line width=0.25pt, black];
\draw [<->] (0.25,-11.8) -- (-0.5,-11.8) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-0.11,-11.55) {$\mathrm{w_{hol}}$};


\draw [<->] (-2.75,-3) -- (-2.75,-4.325) [-stealth, line width=0.25pt, black];
\draw [<->] (-2.75,-4) -- (-2.75,-1.9) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-2.8,-3.35) {$\mathrm{f}$};

\draw [<->] (-2.75,-5) -- (-2.75,-9) [-stealth, line width=0.25pt, black];
\draw [<->] (-2.75,-6) -- (-2.75,-4.325) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-2.8,-6.8) {$\mathrm{a}$};

\draw [<->] (-2.75,-10) -- (-2.75,-12.2) [-stealth, line width=0.25pt, black];
\draw [<->] (-2.75,-11) -- (-2.75,-9) [-stealth, line width=0.25pt, black];
\node[black, anchor=base west] at (-2.8,-10.8) {$\mathrm{b}$};


\draw[black] (-1.77,-7.0275)  arc (78:50:1 and 2);
\node[black, anchor=base west] at (-1.7,-7) {$\gamma$};



\draw[black] (0.265,-0.8)  arc (-58:-122:0.5 and 1);
\node[black, anchor=base west] at (-0.5,-1.52) {$\beta$};


\end{tikzpicture}


==> for arxiv 2/figures/imagespread/imagespread.tex <==
 \begin{tikzpicture}[tight background,rotate=-90]

    % define coordinates
    \coordinate (O) at (0,0) ;
    
    % object
    \draw[ultra thick] (-2,-0.5) -- (-2,0.5) ;
    \draw[red!80!black,ultra thick] (4,-1) -- (4,1) ;
    \draw[ultra thick] (4,-2) -- (4,0) ;
    \draw[red!20!blue, ultra thick] (-2,0) -- (-2,-1); 
	\node[below, text width=30,red!20!blue] at (-2.4,-1.7) {``shifted''};
	\node[below, text width=30,red!20!blue] at (-2.1,-1.55) {object};
    \node[above] at (-1.92,0.5) {object};
    \node[above] at (4.2,1.5) {image};
    \node[above,opacity=0.4] at (-1.045,1.35) {B};
    \node[above,opacity=0.4] at (-0.0,1) {$\bigotimes$};
    \node[above,opacity=0.4] at (-0.5,1) {$\bigotimes$};
    \node[above,opacity=0.4] at (-1,1) {$\bigotimes$};
    \node[above,opacity=0.4] at (-1.5,1) {$\bigotimes$};


    % axis
    \draw[dash pattern=on5pt off3pt] (-2,0) -- (4,0) ;
    \draw[<->] (0,-2) -- (0,2) ;
    \node[right] at (-0.12,2) {TL11};

    % rays
    \draw[red!80!black] (-2,0.5) -- (0,0.5);
    \draw[red!80!black] (-2,0.5) -- (0,0.75);
    \draw[red!80!black] (-2,-0.5) -- (0,-0.5);
    \draw[red!80!black] (-2,-0.5) -- (0,-0.25);
    
    \draw[thick] (-2,0.5) parabola (0,1);
    \draw[thick] plot[smooth,domain=-2:0] (\x, {0.75+0.25/2*\x+0.125*(\x+2)*(\x+2)});
    \draw[thick] (-2,-0.5) parabola (0,0);
    \draw[thick] plot[smooth,domain=-2:0] (\x, {-0.25+0.25/2*\x+0.125*(\x+2)*(\x+2)});
    
    \draw[red!20!blue] (-2,0) -- (0,1);
    \draw[red!20!blue] (-2,0) -- (0,1.25);
    \draw[red!20!blue] (-2,-1) -- (0,0.25);
    \draw[red!20!blue] (-2,-1) -- (0,0);
    
    \draw[thick] (0,1) -- (4,0);
    \draw[thick] (0,1.25) -- (4,0);
    \draw[thick] (0,0.25) -- (4,-2);
    \draw[thick] (0,0) -- (4,-2);
    
    \draw[red!80!black] (0,0.5) -- (4,-1);
    \draw[red!80!black] (0,0.75) -- (4,-1);
    \draw[red!80!black] (0,-0.5) -- (4,1);
    \draw[red!80!black] (0,-0.25) -- (4,1);

    % angles
 %   \draw (0,1) arc (90:130:1);
 %   \draw (0,-1.4) arc (270:290:1.4) ;
 %   \node[] at (280:1.8)  {$\theta_{2}$};
 %   \node[] at (110:1.4)  {$\theta_{1}$};

\end{tikzpicture}

==> for arxiv 2/figures/raypaths/raypaths.tex <==
\subfloat[Standard imaging mode with excited objective lens \label{fig:Image mode ol on}]{
%Matrix Optics Diff non OL.py

\begin{tikzpicture}[yscale=0.5, xscale=0.75]



\def\s{0.7}

\def\nub{5}

%\draw [help lines] (-5,3) grid (5,-5);

\def\xa{1}
\def\xb{0}
\def\xc{-1.5}
\def\xd{-6.5}
\def\xe{-8.5}


% 0 beam

\draw [black,opacity=.7, thick,rounded corners=8pt ] (0,\xa) -- (0,\xb) -- (0,\xc) -- (0,\xd) -- (0,\xe);
\draw [black,opacity=.7, thick,rounded corners=8pt ] (0.5,\xa) -- (0.5,\xb) -- (0.5,\xc) -- (-2,\xd) -- (1,\xe);



%+1 beam 

\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0,\xb) -- (0.40192378864668404,\xc) -- (-0.26794919243112275,\xd) -- (0,\xe);
\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0.5,\xb) -- (0.90192378864668399,\xc) -- (-2.2679491924311224,\xd) -- (1.0,\xe);


%+2 beam 

\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0,\xb) -- (0.8660254037844386,\xc) -- (-0.57735026918962573,\xd) -- (0.0,\xe);
\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0.5,\xb) -- (1.3660254037844386,\xc) -- (-2.5773502691896262,\xd) -- (1.0,\xe);


%objective lens

\fill[gray,opacity=.5] (-3,\xc+0.05)  arc (180:-180:3 and 0.3);

	% Schrift

\node[color=red!80!black, anchor=base west] at (-4.25,\xc+0.5+0.05) {objective lens} ;


% transfer system

\fill[gray,opacity=.5] (-5,\xd+0.5) -- (5, \xd+0.5) -- (5, \xd-0.5) -- (-5, \xd-0.5) -- (-5, \xd+0.5)   ;

	% Schrift

\node[color=red!80!black, anchor=base west] at (0.5,\xd+0.7) {transfer system} ;


%Specimen 
\fill[gray,opacity=.7] (-2,\xb+0.05)   rectangle (2,\xb-0.05) ;
\draw [black,opacity=.7, thick,dotted] (-5,0) -- (5,0);
	% Schrift
\node[color=red!80!black, anchor=base west] at (0.5,\xb+0.2) {specimen plane} ;

%image Plane

\draw [black,opacity=.7, thick,dotted] (-5,\xe) -- (5,\xe);
	% Schrift
\node[color=red!80!black, anchor=base west] at (-4.25,\xe+0.2) {image plane} ;

\end{tikzpicture}

}\hfill{}\subfloat[Imaging mode without objective lens \label{fig:Image mode ol off}]{
%werte aus Matrix Optics Diff non OL.py

\begin{tikzpicture}[yscale=0.5, xscale=0.75]



\def\s{0.7}

\def\nub{5}

%\draw [help lines] (-5,3) grid (5,-5);

\def\xa{1}
\def\xb{0}
\def\xc{-1.5}
\def\xd{-6.5}
\def\xe{-8.5}


% 0 beam

\draw [black,opacity=.7, thick,rounded corners=8pt ] (0,\xa) -- (0,\xb) -- (0,\xc) -- (0,\xd) -- (0,\xe);
\draw [black,opacity=.7, thick,rounded corners=8pt ] (0.5,\xa) -- (0.5,\xb) -- (0.5,\xc) -- (0.5,\xd) -- (-0.15385118347064208,\xe);
 

%+1 beam 

\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0,\xb) -- (0.40192378864668404,\xc) -- (1.7416697508022976,\xd) -- (0,\xe);
\draw [red!40!black,opacity=.7, thick,rounded corners=6pt ] (0.5,\xb) -- (0.90192378864668399,\xc) -- (2.2416697508022976,\xd) -- (-0.1538687033602999,\xe);


%+2 beam 

\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0,\xb) -- (0.8660254037844386,\xc) -- (3.7527767497325675,\xd) -- (0,\xe);
\draw [red!80!black,opacity=.7, thick,rounded corners=4pt ] (0.5,\xb) -- (1.3660254037844386,\xc) -- (4.2527767497325675,\xd) -- (-0.1538889335863205,\xe);


%objective lens

\fill[gray,opacity=.15] (-3,\xc+0.05)  arc (180:-180:3 and 0.3);

	% Schrift

\node[color=red!80!black, anchor=base west] at (-4.25,\xc+0.5+0.05) {objective lens} ;

% transfer system

\fill[gray,opacity=.5] (-5,\xd+0.5) -- (5, \xd+0.5) -- (5, \xd-0.5) -- (-5, \xd-0.5) -- (-5, \xd+0.5)   ;

	% Schrift

\node[color=red!80!black, anchor=base west] at (-4.25,\xd+0.7) {transfer system} ;



%Specimen 
\fill[gray,opacity=.7] (-2,\xb+0.05)   rectangle (2,\xb-0.05) ;
\draw [black,opacity=.7, thick,dotted] (-5,0) -- (5,0);
	% Schrift
\node[color=red!80!black, anchor=base west] at (0.5,\xb+0.2) {specimen plane} ;

%Image Plane

\draw [black,opacity=.7, thick,dotted] (-5,\xe) -- (5,\xe);
	% Schrift
\node[color=red!80!black, anchor=base west] at (-4.25,\xe+0.2) {image plane} ;
\end{tikzpicture}

}


